Random Gossip Processes in Smartphone Peer-to-Peer Networks

In this paper, we study random gossip processes in communication models that describe the peer-to-peer networking functionality included in standard smartphone operating systems. Random gossip processes spread information through the basic mechanism of randomly selecting neighbors for connections. These processes are well-understood in standard peer-to-peer network models, but little is known about their behavior in models that abstract the smartphone peer-to-peer setting. With this in mind, we begin by studying a simple random gossip process in the synchronous mobile telephone model (the most common abstraction used to study smartphone peer-to-peer systems). By introducing a new analysis technique, we prove that this simple process is actually more efficient than the best-known gossip algorithm in the mobile telephone model, which required complicated coordination among the nodes in the network. We then introduce a novel variation of the mobile telephone model that removes the synchronized round assumption, shrinking the gap between theory and practice. We prove that simple random gossip processes still converge in this setting and that information spreading still improves along with graph connectivity. This new model and the tools we introduce provide a solid foundation for the further theoretical analysis of algorithms meant to be deployed on real smartphone peer-to-peer networks. More generally, our results in this paper imply that simple random information spreading processes should be expected to perform well in this emerging new peer-to-peer setting.

==> dcoss 2019 -- full version/amtm.tex <==
\subsection{The Asynchronous Mobile Telephone Model}

Since the pattern of communication in the asynchronous setting can be complex, our first goal in creating our new abstraction is to impose a simple but flexible structure for how processes communicate with each other. To this end, we introduce a meta-algorithm that is run by each process individually, independent of all others processes in the network. This allows us to analyze the running time of a particular instance of an algorithm and, from there, the performance of the algorithm across all concurrent network instances.

We will require two primary properties from our algorithmic structure. First, for our protocols to be truly asynchronous, they will not be able to follow a static procedural flow. Namely, after perfoming some action, an algorithm in this model may have to wait an indeterminate amount of time before performing another action or even being notified of the results of the first action. While we can parameterize an upper bound for this delay in the model for the sake of our analysis, it is unrealistic for an instance of the algorithm to be aware of this parameter. Second, we would like to abstract away the details of the asynchronous communication from the specfics of the algorithm, allowing us to keep our algorithm descriptions as simple as possible.
\begin{algorithm}
\caption{The Asynchronous MTM Interface}
\label{alg:amtm}
% -------------------------------------------------------
\begin{algorithmic}[1]
\State
\State \underline{Initialization:}
\State
\State $neighbors \gets [:]$
\State $state \gets$ {\tt idle}
\State $receiver \gets$ {\tt null}
\State \textproc{Initialize()}
\State
\While{{\tt true}}
\State
\State $tag \gets$ \textproc{GetTag}()
\State {\tt update}($tag$)
\State
\State $neighbors\gets$ {\tt blockForNeighborUpdates}()
\State
\State $receiver \gets$ \textproc{Select}($neighbors$)
\If{$receiver\neq {\tt null}$}
		\State $state \gets$ {\tt blockForConnection}($receiver$)
		\EndIf
\State
\If{$state$ = {\tt connected}}
\State \textproc{Communicate}($receiver$)
\State $state \gets$ {\tt idle}
\EndIf
\EndWhile
\end{algorithmic}
% -------------------------------------------------------



\end{algorithm}

We accomplish both of these goals by implementing a structure that resembles a looped synchronous algorithm but regulates its execution through access to data members that are updated asynchronously. Formalized in Algorithm \ref{alg:amtm}, the protocol initializes three fields:
\begin{itemize}
\item $neighbors$: A key-value store of references to neighboring processes whose advertisements have been received along with their advertisement tags. This set is maintained asynchronously by the model and updated whenever a new advertisement is received. Whenever a new advertisement is received, it replaces the last known advertisement for the corresponding neighboring process.
\item $state$: An enumerated type field chosen from the set $\{{\tt idle}, {\tt connected}\}$. Also modified asynchronously by the model, this field signifies the current progress in any connections the process is involved in.
\item $receiver$: A nullable reference to a single neighbor for communication purposes after a connection is formed.
\end{itemize}
While these fields accomplish our first goal of enabling our algorithms to execute asynchronously, we satisfy our second goal of abstracting communication details from the implementing algorithm by exposing an interface of four functions:
\begin{itemize}
\item \textproc{Initialize}(): Initialization of algorithm-specific data.
\item \textproc{GetTag}(): Return the advertisement tag for this process which is then broadcast to all neighboring processes.
\item \textproc{Select}($neighbors$): Return a neighbor (or {\tt null} for no neighbor) to connect to from among those discovered.
\item \textproc{Communicate}($receiver$): Perform a bounded amount of communication with selected neighbor $receiver$.
\end{itemize}
The execution of an iteration of the algorithm loop begins by getting the process' advertisement tag and broadcasting it to all neighboring processes. The model then blocks until a reference to a neighboring process is added to the $neighbors$ set. Once the $neighbors$ set contains at least one neighbor, the implementing algorithm selects one neighbor from the set and returns it. If the selected neighbor isn't {\tt null}, the protocol then attempts to connect with the selected neighbor, and blocks for another indeterminate duration of time for the connection attempt to succeed $(state\gets {\tt connected})$ or fail $(state\gets {\tt idle})$. If the connection succeeds, the two connected processes communicate before proceeding to the next iteration.

We assume that each step of the protocol executes instantly with the exception of the model functions {\tt blockForNeighborUpdates}() and {\tt blockForConnection()} and the algorithm function \textproc{Communicate}($receiver$). These functions implicitly block the protocol's execution. The model functions block the execution until the $neighbors$ and $state$ fields are available to be referenced by the algorithm, respectively, while \textproc{Communicate}($receiver$) stalls until the connected nodes communicate. In order for this abstraction to be useful to our analysis, however, we need to parameterize the maximum duration of these blocking events. We therefore define the corresponding model parameters $\delta_{update}$, $\delta_{connect}$, $\delta_{comm}$, and $\delta_{old}$ which are not known in advance and can change between executions:
\begin{itemize}
\item $\delta_{update}$: If a process $u$ calls {\tt update}($tag$) at time $\delta$, $u$ will be added to the $neighbors$ set of all neighboring processes by time $\delta + \delta_{update}$ at the latest. This is the maximum time for step 14 of the protocol.
\item $\delta_{old}$: Conversly, if a process $u$ calls {\tt update}($tag$) at time $\delta$, no neighboring process will add $u$ to their neighbors set after time $\delta_{old}$ where $\delta_{old} > \delta_{update}$.
% Intuitively, this means that there is at most a delay of $\delta_{update}$ after $u$ sends an advertisement before it is heard by all its neighbors. More formally, in the context of algorithm, it means that the loop from lines from a neighboring process is heard
\item $\delta_{connect}$: If a process $u$ calls {\tt connect}($v$) at time $\delta$, by time $\delta + \delta_{connect}$ at the latest, either the connection attempt will have failed or $u$ and $v$ will have succesfully connected. This is the maximum time for step 18 of the protocol.
\item $\delta_{comm}$: As stated in the model description, once a connection is formed, the connected processes may engage in a bounded amount of communication, $\delta_{comm}$ defines the maximum time required for this communication to occur. This is the maximum time for step 21 of the protocol.
\end{itemize}

Notice that the specified model only defines how to attempt outgoing connections. While this abstraction is similar to the mobile telephone model in that it restricts a process to one such connection attempt at a time, it will deviate slightly by allowing a single incoming connection attempt as well. This allowance will ease our analysis of algorithms in this setting as it frees a process to accept an incoming connection attempt regardless of its current state. For now, we will assume the process of accepting incoming connection attempts is simply to accept the first connection attempt received and call \textproc{Communicate}($sender$) where $sender$ is the source of the incoming connection.

% The asynchronous mobile telephone model (aMTM) directly describes
% the peer-to-peer interface provided by iOS devices. In this model, nodes can make a variety of function calls to the model however some functions require the node to have access to a prerequisite object in order to call them. Furthermore, nodes must also react to events initiated by the model at any time and therefore must implement a number of callback functions. These functions provide various resources to the node, including in some cases the previously mentioned prerequisite objects needed for making particular function calls. The model assumes the definitions of $\delta_{a}$, $\delta_{f}$, $\delta_{i}$, $\delta_c$, $\delta_s$, and $\delta_d$ are not known in advance and can change from execution to execution.
% \subsubsection{Prerequisite Objects}
% The two types of prerequisite objects are the $invitation$ and $connection$ objects. These objects are both delivered by callback functions implemented by the node and provide access to a number of fields and functions the node may use:
% \begin{itemize}
% \item An \textbf{invitation} object $invite$ is created when there are two nodes $u$ and $v$ such that $u$ calls $Invite(v,info)$ for some context $info$. This object is delivered to $v$ through the $ReceiveInvite(invite)$ callback. The invitation object consists of two attributes, $invite.user$ and $invite.info$, which are references to the node that sent the invitation $u$ and the context information $info$, respectively. It exposes two methods: $invite.Accept()$ and $invite.Reject()$.
% \begin{itemize}
% \item $invite.Accept()$: Accepts the invitation represented by the invitation object $invite$ and will eventually trigger the $InviteAccepted(invite)$ for the node that sent the invitation and the $Connected(conn)$ callback for both the node that sent the invitation and the node that accepted it
% \item $invite.Reject()$: Rejects the invitation represented by the invitation object $invite$ and will eventually trigger the $InviteRejected(invite)$ callback for the node that sent the invitation
% \end{itemize}
% \item A \textbf{connection} object $conn$ is created when there are two nodes $u$ and $v$ such that $u$ calls $AcceptInvite(invite)$ for some invitation object $invite$ where $invite.user = v$. This object is delivered to both $u$ and $v$ through the $Connected(conn)$ callback and consists of a single attribute $conn.user$ which provides $u$ with a reference to $v$ and vice versa. It exposes two methods: $conn.SendData()$ and $conn.Disconnect()$.
% \begin{itemize}
% \item $conn.SendData(data)$: Sends a data resource $data$ to the connected neighbor $conn.user$ after a connection is formed and will eventually trigger the $ReceiveData(conn, data)$ callback for the node $conn.user$
% \item $conn.Disconnect()$: Terminates the connection with neighbor $conn.user$ and will eventually trigger the $Disconnected(conn)$ callback for both connected nodes.
% \end{itemize}
% \end{itemize}
% Notice that while functions called by a particular node that require prerequisite objects are written as methods of the objects, callback functions that require these objects are treated as functions of the model that take the object as a parameter. While functions such as $InviteAccepted(invite)$ and $ReceiveData(conn, data)$ could be expressed as $invite.Accepted()$ and $conn.ReceiveData(data)$ since they depend on $invite$ and $conn$, respectively, the above notation simplifies the interface that must be implemented by each node by only requiring a single function to be implemented, not one for each connection object.
% \subsubsection{Model Functions}
% In addition to the above functions that are only available in the presence of the appropriate prerequisite objects, a node executing an algorithm using the aMTM may call the following functions provided by the model at \emph{any} time:
% \begin{itemize}
% 	\item $SetAdv(tag)$: changes the node's advertisement tag to $tag$
% 	\item $Invite(user,info)$: sends a connection invitation to a neighbor node specified by $user$ along with context information $info$ (the latter
% 	detailing, for example, the purpose for the invitation, etc\ldots)
% \end{itemize}
% \subsubsection{Callback Functions}
% In order to notify nodes of changes the aMTM and provide the necessary prerequisite objects, nodes must implement the following callback functions corresponding to the events that may be triggered by the model:
% \begin{itemize}
% \item $AdvTableUpdate(user,tag)$: an update of the neighbor $user$'s advertisement tag is detected where $tag$ is the new value of the advertisement
% \item $ReceiveInvite(invite)$: an invitation object $invite$ is received
% \item $InviteAccepted(invite)$: an invitation object $invite$ is accepted
% \item $InviteRejected(invite)$: an invitation object $invite$ is rejected
% \item $Connected(conn)$: a connection is formed with a neighboring process $conn.user$
% \item $ReceivedData(conn, data)$: a data resource $data$ is received over connection object $conn$
% \item $Disconnected(conn)$: the connection represented by connection object $conn$ is terminated
% \end{itemize}
% \subsubsection{Model Guarantees}
% \noindent The model provides the following guarantees, which among other things, describe how a node can expect callback functions for itself and its neighbors to be triggered after function calls:

% \begin{itemize}

% \item If a node $u$ makes two calls $SetAdv(a_0)$ and $SetAdv(a_1)$ at times $t_0$ and $t_1$, respectively, such that $t_0 < t_1$, no neighboring node will call $AdvTableUpdate(u, a_{0})$ after calling $AdvTableUpdate(u, a_{1})$.
% \item For a sequence of $n$ calls $SetAdv(a_0),\ldots,SetAdv(a_n)$ made by a node $u$ at times $t_0,\ldots,t_n$ such that $t_n < t_0 + \delta_{a}$ and there exists no additional call $SetAdv(a_{n+1})$ at time $t_{n+1}$ such that $t_{n+1} < t_0 + \delta_{a}$, all neighbors will call $AdvTableUpdate(u,a_{i})$ for some $i\in0,\ldots,n$ at time at most $t_0 + \delta_{a}$.
% \item There exists a time $\delta_{f}$ such that $\delta_{f} > \delta_{a}$ and if $u$ calls $SetAdv(a)$ at time $t$ no node will call $AdvTableUpdate(u, a)$ after time $t + \delta_{f}$. 
% \item If a process $u$ calls $Invite(v,i)$ for some neighboring process $v$ and context $i$, $v$ will trigger $ReceiveInvite(invite)$ within at most time $\delta_i$ where $invite.user = u$ and $invite.info = i$. If $v$ calls $invite.Accept()$, $u$ will trigger $InviteAccepted(invite)$ within at most time $\delta_i$.
% \item After  $InviteAccepted(invite)$ is triggered for a node $u$ after some node $v$ accepts an invitation, $u$ and $v$ will trigger $Connected(conn)$ for the corresponding connection object $conn$ within at most time $\delta_c > \delta_i$.

% \item Once a connection object $conn$ is formed for two nodes $u$ and $v$, if $u$ calls $conn.SendData(data)$ for some resource $data$, $v$ will trigger $ReceivedData(conn, data)$ within at most time $\delta_s$.
% \item If a process $u$ calls $conn.Disconnect()$ for some connection object $conn$ and neighbor $v$ such that $conn.user = v$, $u$ and $v$ will trigger $Disconnected(conn)$ in time at most $\delta_d$.
% \item All advertisement tags specified by the parameter $tag$ and context information specified by the parameter $info$ have a maximum number of bits $b_{max}$.
% \end{itemize}

==> dcoss 2019 -- full version/amtmAlgorithm.tex <==
\subsection{The Asynchronous Random Spread Gossip Algorithm}

We now instantiate our algorithm as a particular instance of the asynchronous mobile telephone model protocol by implementing the four functions specified by the interface. First we initialize the token set of the process to contain any tokens it knows. We also instantiate the hash function used for creating the advertisement tags:\\
% The asynchronous random spread gossip algorithm acts on the above model by implementing the required callback functions defined by the interface. The below pseudocode illustrates the node's initialization and interface implementation:\\
\begin{algorithmic}
\Function{Initialize}{}
\State $tokens \gets$ initial tokens (if any) known by $u$
\State $H \gets$ a hash function
\EndFunction
\end{algorithmic}
\bigskip
Next we define the tag function to simply return the hash of the token set that the process knows:\\
\begin{algorithmic}
\Function{GetTag}{}
\State
\Return $H(tokens)$
\EndFunction
\end{algorithmic}
\bigskip
To select a neighbor from those that a process has discovered, the algorithm will first create a filtered set of neighbors to only include those that would be productive to connect to (those neighbors with different token hashes). Then, following the random gossip strategy, it will select one such neighbor uniformly at random. If no productive neighbor exists then the algorithm doesn't select any neighbor and remains idle. Lastly, note that when a productive neighbor is selected, the algorithm clears its set of known neighbors. As we will see in Lemma \ref{lem:fault}, refreshing the set of known nearby processes minimizes the effect of faulty nodes on performance.\\
\begin{algorithmic}
\Function{Select}{neighbors}
\State $productiveNeighbors\gets\emptyset$
\State
\For{$neighbor$ in $neighbors$}
\If{$neighbor.value \neq \textproc{GetTag}()$}
\State $productiveNeighbors.add(neighbor.key)$
\EndIf
\EndFor
\State
\If{$productiveNeighbors \neq \emptyset$}
\State $neighbors \gets [:]$ // remove stale advertisements
\State \text{// chosen uniformly at random}
\State
\Return $receiver \in productiveNeighbors$
\Else \State
\Return {\tt null}
\EndIf
\EndFunction
\end{algorithmic}
\bigskip
Finally, if two processes form a succesful connection, they exchange a single token in the symmetric set difference between their two token sets:\\
\begin{algorithmic}
\Function{Communicate}{$receiver$}
\State $t\gets$ some $t\in (T$ $\Delta$ $receiver.T$)
\State (exchange token $t$)
\EndFunction
\end{algorithmic}
% The above simply initializes the set $neighbors$ which will be used to maintain a dictionary of $node-tag$ pairs for neighboring nodes and their advertisements,  the node's token set to contain the node's only token $t_{u}$, a reference to a neighbor in an outgoing connection, and a flags indicating if the node received a recent invitation or should block the main loop. It also begins advertising a tag that consists of some hash of the token set set (eg. the md5 hash of the concatenation of the ordered tokens) and begins the main thread of the algorithm which will be called the $ConnectLoop$. To process advertisement updates, a node will replace any advertisement previously received for a neighbor node with the latest update:
% \bigskip
% \begin{algorithmic}
% \Function{AdvTableUpdate}{$user,tag$}
% \State $neighbors[user]\gets tag$
% \EndFunction
% \end{algorithmic}
% \bigskip
% In the asynchronous random spread gossip algorithm, nodes will be able to maintain a single incoming and outgoing connection. $ConnectLoop$, illustrated below will drive the outgoing connections created by the node:\\
% \begin{algorithmic}
% \Function{ConnectLoop}{}
% \While{true}
% \State $prodNeighbors\gets \emptyset$
% \For{$neighbor$ in $neighbors$}
% \If{$neighbor[v] \neq hash(tokens)$}
% \State $prodNeighbors.add(neighbor.key)$
% \EndIf
% \EndFor
% \If{$prodNeighbors \neq [] \wedge block = false$}
% \State $block \gets true$
% \State $v \gets$ $v\in prodNeighbors$ \text{// (random)}
% \State $neighbors \gets [:]$
% \State $SendInvite(v, null)$
% \EndIf
% \EndWhile
% \EndFunction
% \end{algorithmic}
% \bigskip
% The above function repeatedly checks if it knows of any neighbors that hold a different token set then itself and, if not, repeats until this condition is met. If it knows at least one neighbor with a different advertisement and token set, it begins by blocking future iterations of the loop until the connection attempt is resolved. It first clears its neighbors set (in an effort to deal with crash failures which will be discusses later) and sends the selected neighbor an invitation to connect (deciding randomly if multiple neighbors meet this condition). This invitation will result in a trigger of either the $InviteRejected(invite)$ callback or the $InviteAccepted(invite)$ and $Connected(conn)$ callbacks. These are illustrated by the below pseudocode:\\
%  \begin{algorithmic}
% \Function{InviteRejected}{$invite$}
% \State $block \gets false$
% \EndFunction
% \bigskip
% \end{algorithmic}
%  \begin{algorithmic}
% \Function{InviteAccepted}{$invite$}
% \State $outgoing\gets invite.user$
% \EndFunction
% \end{algorithmic}
% \bigskip
%  \begin{algorithmic}
% \Function{Connected}{$conn$}
% \If{$outgoing = conn.user$}
% \State $t\gets$ some $t\in tokens$ $\Delta$ $conn.user.tokens$
% \State $conn.Send(t)$
% \EndIf
% \EndFunction
% \end{algorithmic}
% \bigskip
% The above functions describe the behavior where, if a node invites a neighbor to connect and this invitation is rejected, it unblocks the connection loop to try again with a new neighbor when one is found. If the invitation is accepted, a connection will be formed, but first the sending node should remember that this is an outgoing connection so that when the connection is formed, only the originating node sends a token. This allows the node that accepted the invitation to be the one to terminate the connection as illustrated by the callback below:\\
%  \begin{algorithmic}
% \Function{ReceiveData}{$conn, data$}
% \State $tokens = tokens \cup \{data\}$
% \State $conn.Disconnect()$
% \EndFunction
% \end{algorithmic}
% \bigskip
% \begin{algorithmic}
% \Function{Disconnected}{$conn$}
% \If{$outgoing \neq conn.user$}
% \State $invited = false$
% \Else
% \State $outgoing = null$
% \EndIf
% \State $SetAdv(hash(tokens))$
% \State $block \gets false$
% \EndFunction
% \end{algorithmic}
% \bigskip
% The above adds the received token to the token set and immediately terminates the connection, unblocking the connection loop when the connection closes. It also checks if the connection was an outgoing connection, resetting the $outgoing$ field if it was and resetting the $invited$ field if it wasn't. This concludes the implementation regarding outgoing connections. To also maintain an incoming connections, invitations must be processed. When a node receives an invitation, it follows the simple strategy of accepting any invitation as long as it hasn't previously accepted an invitation that is leading to a connection.\\
% \begin{algorithmic}
% \Function{ReceiveInvite}{$invite$}
% \If{$invited = false$}
% \State $invited = true$
% \State $invite.Accept()$
% \Else
% \State $invite.Reject()$
% \EndIf
% \EndFunction
% \end{algorithmic}
% \bigskip
% The rest of the connection is handled in the same way as the outgoing connections by the above function callbacks. The main idea of this algorithm is for nodes to continuously search for neighbors with different token sets, indicated by their advertisement tags, and attempt connections, meanwhile accepting at most one incoming connection.

\subsection{Asynchronous Random Spread Gossip Analysis}
In this section we analyze the above algorithm. We begin with a proof of convergence, showing that in the worst case the asynchronous random spread gossip algorithm spreads all tokens to all nodes in the network in time $\bigO{nk\delta_{max}}$. We then take advantage of the vertex expansion $\alpha$ to demonstrate how it increases the rate at which a single token is spread.

\subsubsection{Proof of Convergence}
We begin our analysis by showing that the asynchronous random spread algorithm spreads all $k$ tokens to the entire network in time at most $\bigO{nk\delta_{max}}$. Firstly, for our analysis of the asynchronous setting, we will have to redefine our notion of the productive subgraph.

\begin{definition}
At time $\delta$, define $G_\delta$ to be the productive subgraph of the network $G=(V,E)$ at this time such that $G_\delta=(V, E_\delta)$ where $E_\delta = \{(u,v): H(u.tokens) \neq H(v.tokens)$ at time $\delta\}$.
\end{definition}

Notice, as in the previous section, we assume the very low probability event of hash collisions do not occur.
That is: $H(u.tokens) = H(v.tokens) \Longleftrightarrow u.tokens = v.tokens$.
With this in mind, we establish our first bound (remember in the following that $\delta_{update}$, $\delta_{connect}$, and $\delta_{comm}$ are the relevant
maximum time bounds---unknown to the algorithm---for key model behavior).

\begin{lemma}
The asynchronous random gossip algorithm takes time $O(nk\delta_{max})$ to spread all tokens where $n$ is the number of nodes in the network, $k$ is the number of tokens to spread, and $\delta_{max}=O(\delta_{update} + \delta_{connect}+\delta_{comm})$ is the maximum amount of time between iterations of the algorithm loop.
\end{lemma}
\begin{proof}
Fix some time $\delta$. Our goal is to show that within the interval $\delta$ to $\delta+\delta_{max}$,
at least one node learns a new token.
Because
this can only occur at most $nk$ times before all nodes know all tokens,
if we can show the above we have established the lemma.

Fix some time $\delta$. Let $G_{\delta}$ be the {\em productive subgraph} (see the above definition) at the beginning of this interval.
  If not all tokens have spread, clearly there exists a node $u$ such that the $deg(u) > 0$ in $G_{\delta}$. 
  
  By the guarantees of the model, 
  by time $\delta' \leq \delta + \delta_{update} + \delta_{connect}+\delta_{comm}$ , $u$ will have heard advertisements from all neighbors in $G_{\delta}$,
  and then subsequently looped back to the top of its main connect loop.
  
  For each neighbor $v$ in $G_{\delta}$, either $u$ adds $v$ to its set, or at some point after $\delta$, $v$ and $u$'s token sets changed
  such that $u.tokens = v.tokens$, preventing $u$ from adding $v$.
  In this case, however, at least one new token was learned by some node and we are done.
  If this is not the case, then $u$ now has a non-empty $productiveNeighbors$ set.
  
  Going forward, let $v$ be the node $u$ randomly chooses from this set. If the connection fails, this indicates that $v$ is involved in another connection with some other node $v'$.
  If the connection is successful, then $u$ and $v$ will exchange a token.
  Either way, a new token is learned by some node in $\{u,v,v'\}$
  in at most another $\delta_{connect}$ time.
  
  The total amount of time for some node to learn something new is in $O(\delta_{update}+\delta_{connect}+\delta_{comm})$, as needed.
  
  \iffalse
   If the invitation is rejected, this indicates that $v$ has already been invited to a connection by another of its neighbors, and is therefore in the process of sending or receiving a new token. Otherwise, the invitation is accepted, and $u$ and $v$ will trade a token after another $\delta_c$ time.
   Either way, some productive connection occurs.
   
   
   continue with the connection process, forming a connection by time $t+\delta_{a}+2\delta_{i} + \delta_{c}$.
\par Once $u$ and $v$ form a connection, they exchange a single token in the set difference of their token sets. This occurs unless either $u$ or $v$ has received a new token in the interval $(t,t+\delta_{a}+2\delta_{i} + \delta_{c})$ such that this new token makes their token sets equal. Otherwise, $u$ sends a token to $v$ or vice versa and the token is received by the receiver by time $t+\delta_{a}+2\delta_{i} + \delta_{c} + \delta_{s}$. $u$ and $v$ then terminate the connection by time $t+\delta_{a}+2\delta_{i} + \delta_{c} + \delta_{s}+\delta_{d}$. Therefore, over the interval $(t, t+\delta_{a}+2\delta_{i} + \delta_{c} + \delta_{s}+\delta_{d} = O(t, t + \delta_{max})$, either $u$ and $v$ exchange a token, or $u$ or $v$ receive a new token in this interval from another of their neighbors.
\par All the above occurs unless $u$ is already in a connection process at time $t$, in which case clearly progress is made in time at most $2\delta_{i} + \delta_{c} + \delta_{s}+\delta_{d}$, showing that for any interval of length $\delta_{max}$, at least one token is received by one node. Since there are $n$ nodes and $k$ tokens, clearly $nk$ of such intervals are required. In the worst case, where none of these $nk$ intervals of length $\delta_{max}$ overlap, the total time required by the algorithm is $O(nk\delta_{max})$.
\fi
\end{proof}



\begin{lemma} \label{lem:fault}
Let $t$ be the maximum number of faulty nodes in the network, the asynchronous random gossip algorithm takes time $O(\delta_{max}(nk+t))$ to spread all tokens.
\end{lemma}
\begin{proof}

Again, consider the productive subgraph $G_{\delta}$ at a particular time $\delta$ for a node $u$ when its $neighbors$ set is empty. If no nodes leave the subgraph then $u$ is guaranteed to learn of all these neighbors and add them to its $neighbors$ set. However, now allow some node $v$ in $u$'s $neighbors$ set to experience a failure between times $\delta-\delta_{old}$ and $\delta+\delta_{max}$ (if the failure happens before $\delta-\delta_{old}$ then by the guarantee of the aMTM, $u$ will not have received $v$'s update). Upon entering an iteration of the outer loop, $u$ may attempt to connect with $v$ since $v$'s advertisement is still fresh. In this event, which is clearly the worst case, the connection fails and time at most $\delta_{max}$ was spent since this is the maximum amount of time the outer loop can possibly take.
\par This failure can happen in each new iteration of the outer loop for at most time $\delta_{old}$, at which point the advertisement ceases to update $u$'s neighbor set. Therefore, a single failed node can cause a delay of time at most $\delta_{old} + 2\delta_{max}$. Since there are $t$ faulty nodes, this introduces a total slowdown of $t(\delta_{old} + 2\delta_{max})$. Therefore, the time for this algorithm to spread all $k$ tokens is $\bigO{nk\delta_{max}} + t(\delta_{old} + \delta_{max})$. Furthermore, if we assume $\delta_{old} = \bigO{\delta_{update}}=\bigO{\delta_{max}}$, $\bigO{nk\delta_{max} + t2\delta_{max}}=\bigO{\delta_{max}(nk+t)}$.
\end{proof}
\begin{lemma}
Let $b$ be the maximum fraction of neighbors for a node $u$ that can be byzantine, the asynchronous random gossip algorithm takes time $O(nk\delta_{max}/(1-b))$ in expectation to spread all tokens.
\end{lemma}
\begin{proof}
If the productive subgraph stays connected, the worst event that can occur during the interval of length $\delta_{max}$ is that an honest node chooses a byzantine neighbor to connect to. This happens with probability at most $b$ and therefore a node engages in a productive, honest connection with probability at least $1-b$. Consider the series $m$ of intervals of time at most $\delta_{max}$ and label them with the indicator variables $X_1,\ldots,X_m$ such that:
\[
X_i =
\begin{cases}
0 &\text{if the node in interval $i$ connects to a}\\ &\text{byzantine node} \\
1 &\text{otherwise }
\end{cases}
\]
\begin{align*}
nk &= E\big[\sum_{i=1}^{i=m}{X_i}\big] \\
&= \sum_{i=1}^{i=m}{E[X_i]} \\
&= \sum_{i=1}^{i=m}{1-b} = m(1-b)
\end{align*}
Therefore, achieving $nk$ successes in expectation, would take $m=\frac{nk}{1-b}$ intervals. Since each interval takes at most $\delta_{max}$ time, the algorithm takes time $O(nk\delta_{max}/(1-b))$.
\end{proof}










\subsubsection{Analysis of Spreading a Single Token}

We now analyze the spread of a single token in the network to demonstrate that the performance of the algorithm still improves with the vertex expansion of the network $\alpha$ in an asynchronous setting. Our goal in this subsection is to prove the following time bound to spread a single token:

\begin{theorem} \label{thm:async}
The asynchronous random spread gossip algorithm takes time at most $\bigO{\delta_{max}\sqrt{n/\alpha}\log^2{(n\alpha)}}$, where $n$ is the number of nodes in the network, $\alpha$ is the vertex expansion, and $\delta_{max}$ is the maximum time required for an iteration of the asynchronous mobile telephone model loop.
\end{theorem}

 Unlike with our analysis of the synchronous algorithm, we cannot directly leverage a productive subgraph that remains stable through synchronized rounds.
We must instead identify cores of useful edges amidst the unpredictable churn and argue that over a sufficiently long interval they deliver a sufficiently large number of new tokens.

%
%
% This is because at a particular time $t$ there is no guarantee that, for all edges $(u,v)\in E_t$,
%that $u$ and $v$ have heard each other's advertisements. To circumvent this issue, we will still fix $G_\delta$ but examine the subgraph of $G_\delta$ that represents only those edges that correspond to the advertisements heard some time within the interval $(\delta, \delta_{update})$. This will allow us to analyze the behavior of the nodes at this time and we return to the entire productive subgraph later.

We accomplish this by fixing the productive subgraph at $G_{\delta}$ and observe an interval of length $2\delta_{max}$. During this interval, we want to show that for every edge $(u,v)\in E_{\delta}$ such that $u$ is informed and $v$ is uninformed, either $v$ becomes otherwise informed or $u$ returns $v$ from \textproc{Select}($neighbors$) with good probability during this interval. Namely, this probability is lower-bounded by the probability $u$ would return $v$ if $neighbors$ included all of $u$'s neighbors from $G_{\delta}$ itself.

\iffalse
\note{The writing for the definition and lemma that follow is clear and good. The subtleties of the timing assumptions, however, seem to be not quite right. A few points on how to fix:
\begin{enumerate}
  \item I don't understand the definition $G^\prime_\delta$. It includes every $v$ from $E_{\delta}$ such that $u$ hears an advertisement from $v$ during an interval of length $\delta_a$.
  By definition of $\delta_a$, however, wouldn't $u$ hear from {\em every} such neighbor in the interval? Meaning that $E'_{\delta}$ always is the same as $E_{\delta}$? I don't think we need
  this definition...
  
  \item To lemma is more or less right, but it's so tricky to capture some of this in words that we need to be careful to be extra clear. Start with time $\delta$. Fix the productive subgraph $G_{\delta}$.
  Here you need to emphasize that for each node $u$ that knows the message their number of uninformed neighbors can only {\em decrease}. This is crucial for your implied assumption that $deg(u)$ upper bounds
  $deg'(u)$.
  Once this is established, you can then move to $\delta + \delta_a$. At this point, $u$ has heard from all neighbors. Next, you need to move to the next time after $\delta + \delta_a$ that $u$
  fills its $prodNeighbors$ set, which occurs by time no later than $\delta + \delta_a + \delta_max$.
  
  \item It is at this point that you can fix $deg'(u)$ and note that it is cannot be larger than $deg(u)$ from the original productive subgraph.
  Therefore, it seems we do not need $G'$ and the lemma can be stated with respect to $u$'s degree in the productive subgraph at $\delta$.
  
  This is basically what you have now. I'm just massaging things for maximal clarity (and removing the new productive subgraph definition)
  
  \item I think the lemma wording also has to be clarified  some because it's not exactly clear what "chooses to connect to" means.
  Say something like: fix $\delta$, fix $G_{\delta}$, fix a $(u,v)$ in this productive subgraph.   At some point between
  $\delta$ and $\delta + O(\delta_{max})$, $u$ will select a connection from a set of size no more than $deg(u)$ that includes $v$.
  (Is ``select a connection" right? Maybe there's an even clearer way of saying this. As long as it's clear and we're consistent...)
  
      
\end{enumerate}
t
}
\begin{definition}
For a fixed time $\delta$ and productive subgraph $G_\delta$, define $G^\prime_\delta=(V,E^\prime_\delta)$ where $E^\prime_\delta=\{(u,v)\in E_\delta:u \text{ receives v's advertisement in the interval }(\delta, \delta+\delta_{update})\}$.
\end{definition}
\fi


\begin{lemma} \label{lem:randomlemma}
% For a fixed time $\delta$ and fixed edge $(u,v)\in E_{\delta}$. Node $u$ returns $v$ from \textproc{Select} with probability at least $deg_\delta(u)$ (where $deg(u)$ is the degree of $u$ in the productive subgraph) and the resulting connection attempt concludes no later than time $\delta+2\delta_{max}$.
For a fixed time $\delta$ and fixed edge $(u,v)\in E_{\delta}$ such that $u$ knows the token and $v$ does not, if $v$ does not otherwise learn the token in this interval, node $u$ returns $v$ from \textproc{Select}($neighbors$) uniformly at random from a set of at most $deg(u)$ nodes where $deg(u)$ is the degree of $u$ in the productive subgraph and the resulting connection attempt concludes no later than time $\delta+2\delta_{max}$.
\end{lemma}

\begin{proof}
Fix the productive subgraph at this time, $G_{\delta}$ and fix an informed node $u$ and uninformed node $v$. Since $u$ is an informed node, all of its edges in the productive subgraph are incident to uninformed nodes. Since nodes never forget the token, the number of uninformed nodes can only decrease. Now consider an execution of \textproc{Select}($neighbors$) before time $\delta + \delta_{max}$ in which $v$ is added to $u.productiveNeighbors$. Since by assumption $v$ does not otherwise learn the token in this interval, it must be the case that $v$ advertised its uninformed status in this interval and been included in $u.neighbors$ and subsequently $u.productiveNeighbors$ so we know this occurs at least once in the interval $\delta + \delta_{max}$ (the extra time $\delta_{connect}+\delta_{comm}$ is to allow an additional iteration of $u$'s loop before \textproc{Select} is called). Furthermore, we know that since the number of uninformed neighbors can't increase from that in the productive subgraph $G_\delta$, there can be at most $deg(u)$ neighbors in $u.productiveNeighbors$. Since $u$ returns a particular neighbor from this set with uniform randomness, the probability that $u$ returns $v$ is at least $1/deg(u)$. Furthermore, regardless whether or not the resulting connection attempt is a success or a failure, it finishes in at most $\delta_{connect}+\delta_{comm}$ additional time for a total maximum time of $\delta_{update}+2(\delta_{connect}+\delta_{comm})<2\delta_{max}$.

\end{proof}
Now that we have quantified the amount of time necessary for a node to successfully connect, we need an estimate for how many connections we can expect to be succesful. Similar to our previous analysis, this is dependent on the amount of competition between connection attempts sent to a single node.
We begin with a useful graph theory definition.
\iffalse
\note{A general stylistic note: You need to introduce definitions and lemmas before they appear. I added some text to this effect below, but in other places where this is missing, you'll want to add it.
I changed the name from {\em weight} to {\em degree weight} below, because you're defining a specific weight based on degree.}
\fi
\begin{definition}
For a graph $G=(V,E)$, we define the \textbf{degree weight} of a node be the sum of the weights of all incoming edges, where the weight of each edge $(u,v)$ is $1/deg(u)$. Formally:
\[w(v)=\sum_{\forall u\in V, (u,v)\in E}w(u,v)=\sum_{\forall u\in V, (u,v)\in E}1/deg(u)\]
\end{definition}

We now prove a useful result about one-round random matchings in a bipartite graph that leverages our degree weight definition in its proof.

\begin{lemma} \label{lem:sqrtlemma}
For a bipartite graph G=(X, Y, E) with edge independence $\edgeindnum{B(X)}=|X| = m$. 
Assume each node $u\in X$ selects a neighbor with uniform randomness with probability $1/deg(u)$. With at least constant probability, at least $\sqrt{m}/\log{m}$ distinct nodes from $Y$ are selected.
\end{lemma}
\begin{proof}
Partition the nodes of $Y$ into a ``core" set of nodes $Z$ with constant degree weight, and a ``non-core" set of nodes $Y \setminus Z$ with less than constant weight. 

We first consider the case where $|Z| \geq \sqrt{m}$. Here it is sufficient to show that nodes with at least constant weight are selected with constant probability. 
For a node $v\in Z$ such that $(u,v)\in E$, the probability that $u$ does not select $v$ is at most $1-1/deg(u)=1-w(u,v)$. Therefore the probability that $v$ is selected by {\em some} node is:
\begin{align*}
\Pr[\text{$v$ is selected}] &\geq 1 - \Pi_{u,(u,v)\in E}(1 - w(u,v))\\
&\geq 1 - \Pi_{u, (u,v)\in E}e^{-w(u,v)}\\
&\geq 1 - e^{-\sum_{u, (u,v)\in E}w(u,v)}\\
&\geq 1 - e^{-w(v)}
\end{align*}
Since by our assumption $w(v)$ is a constant, $v$ is selected with at least constant probability. If we denote this probability $p$, we can express the probability that $v$ is not selected as $1-p$. Therefore, the expected number of nodes in the core set that are not selected is at most $(1-p)\sqrt{m}$. Let $W$ be the number of core nodes that are not selected, we can apply Markov's inequality to demonstrate that the probability we exceed this expectation by more than a constant fraction is at most constant:
\begin{align*}
\Pr[W\geq 2(1-p)\sqrt{m}] \leq \frac{1}{2}
\end{align*}
Therefore, with at least a constant probability, $\bigO{\sqrt{m}}$ nodes are selected from the core set.
% \iffalse
% \note{For the above case, you have established that $v$ is selected with constant probability. But the lemma says that with constant probability, at least $\sqrt{m}$ nodes are selected. So there
% is still work to do to get from your analysis of a single node to the total number of nodes. You can probably apply markov's inequality to bound the number of unselected nodes.

% For the below case, we need a clearer and stronger way of arguing the $1/\sqrt{m}$ selection probability on nodes in $Y \setminus Z$.
% For one thing, it's not true that every node in $X$ selects a node in that set with that probability. Some nodes in $X$ may only have edges to nodes in $Z$.
% I think you mean each node in $Y\setminus Z$ has a degree weight of at least $1/\sqrt{m}$. The argument for this case needs to be more precise some how...

% Also please carefully check that your argument about multiple selections is right. Is it really the case that the probability that the $i^{th}$ node makes an overlapping suggestion 
% is $(i-1)/m$? This implies that each such node is choosing among all $m$ nodes equally doesn't it? Does that hold?}
% \fi

Now consider the case where $|Z|<\sqrt{m}$. Observe that for a node $u\in X$ that neighbors a node in $Y\setminus Z$, the sum of the edge weights for edges $(u,v)$ such that $v\in Y\setminus Z$ is at least $1/\sqrt{m}$. This is because $u$ can select at most $\sqrt{m}-1$ other nodes that are not in $Y\setminus Z$. Therefore, for each node in $X$ that neighbors a node in $Y\setminus Z$, the node in $X$ chooses a node in $Y\setminus Z$ with probability at least $1/\sqrt{m}$. Since there must be $m-|Z|$ such nodes in $X$ that neighbor nodes in $Y\setminus Z$, in expectation at least $\bigO{m/\sqrt{m}}=\bigO{\sqrt{m}}$ nodes in $X$ select a node in $Y \setminus Z$.\\

Next, conditioned on the event that $\sqrt{m}$ nodes from $X$ select non-core nodes, we need to show that not too many of the nodes in $Y \setminus Z$ are chosen multiple times. Namely, we would like to show that the probability that any node is selected by more than $c\log{m}$ nodes (for some sufficiently large constant $c$) from $X$ that choose a non-core node is small. Fix a node $v\in Y$ and define the indicator variable $I_j$ as follows:
\[
X_j =
\begin{cases}
1\text{ the $j$th node in $X$ selects $v$}\\
0\text{ otherwise}
\end{cases}
\]
Since the size of the maximum matching is size $m$ and there are $m$ nodes in $Y$, we know that $v$ has at most constant degree weight and therefore, in expectation, is selected by at most a constant number of nodes from $X$. Denote this constant expectation $\mu$ and apply the following Chernoff bound to the sequence $I_1,\ldots,I_m$ with expectation $\mu$ to upper bound the probability that the total number of such nodes $I=\sum_{j=1}^{m}I_j$ exceeds $c\log{m}$. For a sufficiently large constant $c$ and constant $\mu$ we find that this probability is polynomially-small in $m$:
\begin{align*}
\Pr[I\geq (1+ \epsilon)\mu] &\leq e^{-\frac{\epsilon\mu}{3}} \\
\Pr[I\geq \mu c \log{m}] &\leq e^{-\frac{\mu(c\log{m}-1)}{3}} = \frac{e^{\mu/3}}{me^{c\mu/3}} \leq \frac{1}{m}
\end{align*}
Therefore, if we apply the union bound over the at most $m-\sqrt{m}\leq m$ nodes in $Y\setminus Z$ we can upper bound the probability that any such node is selected by at least $c\log{n}$ nodes in $X$:
\begin{align*}
  \sum_{i\in[m]}\frac{e^{\mu/3}}{me^{c\mu/3}}=m\frac{e^{\mu/3}}{me^{c\mu/3}} < constant
\end{align*}
% can have at most a constant number of nodes.  $u\in X$ for which $v$ is $u$'s only neighbor. Therefore, most nodes in $u\in X$ (any number greater than constant) must have at least one other neighbor besides $v$ in $Y$. Therefore, the probability $u$ selects $v$ is at most $1/2$. Therefore, the probability that at least $c\log{n}$ nodes select $v$ is at most $(1/2)^{m^{1/4}}$. If we apply the foll union bound over all $m$ nodes in $Y\setminus Z$ we can upper bound the probability that any such node is selected by at least $m^{1/4}$ nodes in $X$:
Therefore, with at least constant probability no node is selected by at least $c\log{n}$ nodes from $X$ that choose non-core nodes. Therefore, given that $\sqrt{m}$ nodes select non-core nodes, with at least a constant probability at least $\bigO{\sqrt{m}/\log{m}}$ nodes are selected.
\end{proof}

The above lemmas allow us to quantify the number of successful connections made in an interval of length $\delta_{update}+2\delta_{max}$ with respect to $G_\delta$ for some time $\delta$, but we need to relate this result back to the productive subgraph as a whole.
% \iffalse
% \note{How are you getting high probability below? You want to fix the productive subgraph at $G_{\delta}$ and identify its matching of size $m$.
% You need to then apply the bipartite graph lemma to show that if informed nodes on the frontier properly selected neighbors in the prodcutive subgraph in a synchronized
% way then with constant probability a root-factor would be selected.
% Then you then to connect this to the connection lemma from before, which is the tricky part}
% \fi
\begin{lemma} \label{lem:step}
Fix the productive subgraph $G_\delta$ with a maximum matching of size $m$. With high probability, $\sqrt{m}/\log{m}$ successful connections will occur by time $\delta+ \delta_{update}+2\delta_{max}$.
\end{lemma}

\begin{proof}
For a fixed $G_{\delta}$, if we consider an edge $(u,v)\in E_{\delta}$ consisting of an informed node $u$ and uninformed node $v$ such that $v$ is not otherwise informed in this interval, we know from Lemma \ref{lem:randomlemma} that $u$ adds $v$ to $u.productiveNeighbors$ some time before $\delta+\delta_{update}+\delta_{max}$. Since $u$ returns $v$ from \textproc{Select}($neighbors$) with probability at least $1/deg(u)$, inclusion of $v$ in $u.produtveNeighbors$ represents a selection weight of at least $1/deg(u)$ for the edge $(u,v)$. Since the selection weight for this edge never decreases, the edge weight for $(u,v)$ accumulated in this interval (and therefore its selection probability) must be at least $1/deg(u)$ (the weight the edge would have in the productive subgraph itself). Therefore, the collection of these edge weights observed over this interval represents a bipartite graph with maximum matching of size $m$ where each edge is selected with probability at least $1/deg(u)$. Therefore, according to Lemma \ref{lem:sqrtlemma}, with at least constant probability, $\sqrt{m}/\log{m}$ nodes are selected over this interval. Furthermore, each connection attempt takes at most $\delta_{max}$ time which concludes our Lemma as long as Lemma \ref{lem:randomlemma} holds.

However, since Lemma \ref{lem:randomlemma} assumes that for each of these productive edges $(u,v)$, $v$ is not otherwise informed, we must consider this case as well. However, since $(u,v)\in E_{\delta}$ and $v$ can only have been informed through a prior successful connection during this interval, it should be clear that this event does not reduce the number of successful connections that take place during this interval and so the Lemma is still satisfied.
\end{proof}
To continue our analysis with respect to the vertex expansion, we now relate the expected number of productive connections at fixed points in time to the $\alpha$.
\begin{lemma} \label{lem:constantfraction}
Let $S(\delta)$ be the subset of informed nodes such that $n(\delta)=|S(\delta)|$ and $n^*_\delta=\min(|S(\delta)|, |V\setminus S(\delta)|)$. Furthermore, abbreviate $\delta_{update}+2\delta_{max}$ to $\delta_{interval}$. With high probability, if $n(\delta) \leq n/2$, it takes at most time $2\delta_{interval}\log{(n(\delta)\alpha)}\sqrt{n(\delta)/\alpha}$ to at least double the number of informed nodes. Explicitly, with high probability: $$n(\delta + 2\delta_{interval}\log{(n(\delta)\alpha)}\sqrt{n(\delta)/\alpha})\geq 2n(\delta)$$
\end{lemma}

\begin{proof}
Consider a sequence of fixed times $\delta_0,\ldots,\delta_t$ that are time $\delta_{interval}$ apart. Lemma \ref{lem:step} estimates the number of succesful connections with respect to the size of the maximum matching while Lemma \ref{lem:msize} which relates the size of the maximum matching size $m$ to the vertex expansion such that $m\geq n(\delta)\alpha$ for $0<n(\delta)\leq n/2$. Therefore, with high probability, the number of nodes that become informed between $\delta_{i-1}$ and $\delta_i$ is $n(\delta_{i-1}) + (1/2)\sqrt{n(\delta_{i-1})\alpha}/\log{(n(\delta_{i-1})\alpha)}$. Therefore, the number of nodes that are informed by time $\delta_t$ is: $$n(\delta_t)=n(\delta_0)+(1/2)\sqrt{n(\delta_{0})\alpha}/\log{(n(\delta_{0})\alpha)}+\ldots$$
$$\ldots+(1/2)\sqrt{n(\delta_{t-1})\alpha}/\log{(n(\delta_{t-1})\alpha)}$$
Since clearly $n(\delta_j)\geq n(\delta_{i})$ for any $j\geq i$, we can simplify the above:
$$n(\delta_t)\geq n(\delta_0) + (t/2)\sqrt{n(\delta_{0})\alpha}/\log{(n(\delta_{0})\alpha)}$$
Lastly, if we set $n(\delta_t)=2n(\delta_0)$ we can solve for $t$:
\begin{align*}
2n(\delta_0) &\geq n(\delta_0) + (t/2)\sqrt{n(\delta_{0})\alpha}/\log{(n(\delta_{0})\alpha)}\\
n(\delta_0) &\geq  (t/2)\sqrt{n(\delta_{0})\alpha}/\log{(n(\delta_{0})\alpha)}
\end{align*}
\[2\log{(n(\delta_{0})\alpha)}\sqrt{n(\delta_{0})/\alpha} \geq  t \]

Since there are most $2\log{(n(\delta_{0})\alpha)}\sqrt{n(\delta_{0})/\alpha}$ steps of length $\delta_{interval}$, the total time to double the number of informed nodes from $n(\delta_0)$ is at most $2\delta_{interval}\log{(n(\delta_{0})\alpha)}\sqrt{n(\delta_{0})/\alpha}$.
 % a sequence of timesteps $\delta0,\ldots,\delta_{\sqrt{n/\alpha}}$, such that $\delta_{i+1}=\delta_{i} +\delta_{update}+2\delta_{max}$ for $i\in\{0,\ldots,\sqrt{n/\alpha}-1\}$, we know from Lemma \ref{lem:step} that with high probability $n^*(\delta_{i+1}) = n^*(\delta_{i}) + \sqrt{\alpha n^*(\delta_i)/4})$. Therefore, again with high probability, $n^*(\delta^\prime) = n^*(\delta_{0}) + \sqrt{\alpha n^*(\delta0)/4}) + \ldots + \sqrt{\alpha n^*(\delta_{\sqrt{n/\alpha}-1})/4})$. Furthermore, since $n^*(\delta_{i+1}) \geq n^*(\delta_{i})$, $n^*(\delta^\prime)\geq n^*(\delta_{0}) + \sqrt{n/\alpha}\cdot\sqrt{\alpha n^*(\delta0)/4})\geq (5/4)n^*(\delta0)$.
\end{proof}
We now use the length of this interval to analyze the time required to spread the token to half of the nodes in the network.
\begin{lemma} \label{lem:half}
It takes time at most $\bigO{\delta_{max}\sqrt{n/\alpha}\log^2{(n\alpha)}}$ to spread the token to $n/2$ nodes in the network.
\end{lemma}
\begin{proof}
By Lemma \ref{lem:constantfraction}, we can see that if there $n(\delta)$ informed nodes for a given time $\delta$, after time $2\delta_{interval}\log{(n(\delta)\alpha)}\sqrt{n(\delta)/\alpha}$, with high probability we at least double the number of informed nodes. Therefore, to find the number $t$ of intervals required, it suffices to solve for $T$ such that:
\[2^{T-1}=n/2\]
Which yields $T=\log{n}$. Therefore, since each interval takes time at most $\bigO{\delta_{interval}\sqrt{n/\alpha}\log{(n\alpha)}}=\bigO{\delta_{max}\sqrt{n/\alpha}\log{(n\alpha)}}$, the total time required is $\bigO{\delta_{max}\sqrt{n/\alpha}\log^2{(n\alpha)}}$.
% Since $2^{i-1}$ nodes know the token at time $i-1$, step $i$ takes time $2\delta_{interval}\sqrt{2^{i-1}/\alpha}$. Therefore, the total time to spread to $n/2$ nodes is:
% \begin{align*}
% \sum_{i=0}^{\log{n} - 1}2\delta_{interval}\sqrt{2^i/\alpha} &= \frac{2\delta_{interval}}{\sqrt{\alpha}}\sum_{i=0}^{\log{n} - 1}\sqrt{2}^i \\
% &= \frac{2\delta_{interval}}{\sqrt{\alpha}}\frac{1-\sqrt{2}^{\log{n}}}{1 - \sqrt{2}}\\
% &= \frac{2\delta_{interval}}{\sqrt{\alpha}}\frac{\sqrt{2}^{\log{n}}-1}{\sqrt{2}-1} \\
% &= \bigO{\sqrt{2}^{\log{n}}/\sqrt{\alpha}} \\
% &= \bigO{{2^{\log{n}}}^{1/2}/\sqrt{\alpha}} \\
% &= \bigO{n^{1/2}/\sqrt{\alpha}} \\
% &= \bigO{\sqrt{n/\alpha}}
% \end{align*}
\end{proof}
We now have all the necessary components to prove our main theorem about the time required to spread the token to all nodes in the network.
\begin{proof} [Proof (of Theorem~\ref{thm:async})]
When $n(\delta) > n/2$, our goal is to reduce the number of uninformed nodes by half. However, we can no longer relate the size of the maximum matching to the number of informed nodes since we are instead limited by the uninformed nodes since $|V\setminus S_\delta| < |S_\delta|$. Therefore, for fixed times $\delta_0,\ldots,\delta_t$ which are $\delta_{interval}$ apart, we can express the number of uniformed nodes at time $\delta_t$, $n^*({\delta_t})$, as:
$$n^*(\delta_t)=n^*(\delta_0)-(1/2)\sqrt{n^*(\delta_{0})\alpha}/\log{(n^*(\delta_{0})\alpha)}-\ldots$$
$$\ldots-(1/2)\sqrt{n^*(\delta_{t-1})\alpha}/\log{(n^*(\delta_{t-1})\alpha)}$$
Setting $n^*({\delta_t})=n^*({\delta_0})/2$ and solving for $t$ yields:
$$n^*(\delta_0)/2 =n^*(\delta_0)-(1/2)\sqrt{n^*(\delta_{0})\alpha}\log{(n^*(\delta_{0})\alpha)}-\ldots$$
$$\ldots-(1/2)\sqrt{n^*(\delta_{t-1})\alpha}/\log{(n^*(\delta_{t-1})\alpha)}$$
$$\geq (t/2)\sqrt{n^*(\delta_{t-1})\alpha}/\log{(n^*(\delta_{t-1})\alpha)}$$

Which shows that $t\leq 2\sqrt{n(\delta_{t-1})/\alpha}\log{(n(\delta_{t-1})/\alpha)}$, similar to Lemma \ref{lem:constantfraction}. We can apply a proof symmetric to that of Lemma \ref{lem:half} to relate this time to the time to spread the token to all the remaining $n/2$ nodes. Observe that again we need $T=\log{n}$ intervals of length $2\delta_{max}\sqrt{n^*(\delta)/\alpha}\log{(n^*(\delta)\alpha)}$ since we are halving the number of uniformed nodes each time. Therefore, the total time once again is $\bigO{\delta_{max}\sqrt{n/\alpha}\log^2{(n\alpha)}}$ to spread the token to all remaining nodes. Therefore, the total running time of the algorithm is $\bigO{\delta_{max}\sqrt{n/\alpha}\log^2{(n\alpha)}}$.
% Look at matching at the matching of the productive subgraph limite by the n /2 nodes.
\end{proof}
% \iffalse
% \subsubsection{Analyis of Spreading $k$ Tokens}
% For this analysis, we define the productive subgraph with the same definition as Definition $\ref{def:asynchsubgraph}$ and use the same notation as in Section \ref{f}.
% \begin{lemma}
% Let $G_{\delta1,\delta2}$ be the productive subgraph during this interval and define $G^\prime_{\delta1,\delta2}$ as follows:
% \begin{itemize}
%     \item $G^\prime_{\delta1,\delta2}=(G^\prime_{\delta1,\delta2},V^\prime_{\delta1,\delta2}, E^\prime_{\delta1,\delta2})$
%     \item $V$ = $\{(u, r): u\in V, r\in u.tokens \text { or } r\in v.tokens \text{ for some  } v\in N(r)\}$
%     \item $E$ = $\{((u, r), (v, r)): u\in V, v\in V, r\in v.tokens$ and $r\notin u.tokens$ or $r\in u.tokens$ and $r\notin v.tokens$
% \end{itemize}
% The vertex expansion of $G^\prime_{\delta1,\delta2}$ is $\alpha$ where $\alpha$ is the vertex expansion of $G_{\delta1,\delta2}$.
% \end{lemma}
% \begin{proof}
% For each edge $(u,v)$ in $G_{\delta1,\delta2}$, by the definition of the productive subgraph $u.tokens \neq v.tokens$. By the definition of $G^\prime_{\delta1,\delta2}$, for each token that is missing from $u.tokens$ or $v.tokens$ and is present in the other node, there is a copy of both nodes, connected to all copies of both nodes. This creates a bipartite graph where every node of one partition is connected to every node of the other. The vertex expansion of this subgraph is 1, since choosing any less than all the copies of one partition yields a vertex expansion of greater than 1. Therefore, by replacing all such edges in the productive subgraph with these connected components, the vertex expansion of this new graph is also $\alpha$.
% \end{proof}
% \begin{lemma}
% The asynchronous random spread gossip algorithm takes time at most $\bigO{k\sqrt{n/\alpha}\log{n}}$ to spread all $k$ tokens to all $n$ nodes in the network.
% \end{lemma}
% \begin{proof}
% The analysis of the $k$-token case is analagous to that of the single token case except for the length of the intervals required to spread to a number of nodes equal to a constant fraction of the number of current informed nodes. This is because, in $G^\prime_{\delta1,\delta2}$, we must spread to $\bigO{kn}$ nodes but in each interval of length $\delta_{update} + 2\delta_{max}$ we still only make progress of $\bigO{\sqrt{\alpha n}}$ with high probability. Therefore, it takes time at most $\bigO{k\sqrt{n/\alpha}}$ to spread to a constant number of node-token pairs, and through a similar proof to the previous subsection, we get a total time of $\bigO{k\sqrt{n/\alpha}\log{n}}$.
% \end{proof}
% This bound outperforms the trivial bound for any $\alpha > 1/n$ and achieves a running time of $\bigO{n^{3/2}\log{n}}$ for very well-connected graphs.
% Lastly, since we proved in Section \ref{sec:warmup} that the running time is $\bigO{n^2}$, we are free to express the running time of this algorithm as $\min(\bigO{n\sqrt{n/\alpha}\log{n}}, \bigO{n^2}).$
% \fi

==> dcoss 2019 -- full version/asynchGossip.tex <==

\section{Random Gossip in the Asynchronous Mobile Telephone Model}
\label{sec:amtm}

% \textbf{Analysis}
% First we recall some preliminaries. Let $G=(V,E)$ be an undirected graph such that $n=|V|$. For a vertex $u\in V$, define the \textit{neighbors} of $u$ as $N(u)=\{v\in V:(u,v)\in E\}$ and for any subset of vertices $S\subseteq V$, define the \textit{boundary} of $S$ as $\boundary{S}=\bigcup_{u\in S}N(u)\setminus S$, namely, $\boundary{S}$ is the set of all vertices directly adjacent to vertices in $S$, excluding any vertices in $S$ itself. The \textit{vertex expansion} $\alpha$ of the graph $G$ is then defined as:
% \[\alpha=\min_{S\subset V,0<|S|\leq n/2}=\frac{\boundary{S}}{|S|}\]
% Let $B(S)$ denote the bipartite graph $B(S)=(S, V\setminus S, \{(u,v)\in E: u\in S, v\in V\setminus S\})$. We then denote the size of the maximum matching on $B(S)$ the (ie. the \textit{edge independence number}) by $\edgeindnum{B(S)}$.\\

% We then introduce some useful notation. Let $u\in V$ be a node in $G$ and denote $u$'s advertisement at time $\delta$ as $a_u(\delta)$. Next we denote the \textit{productive neighbors} of $u$ at time $\delta$ as $N^*_u(\delta)=\{v\in N(u): a_u(\delta)\neq a_v(\delta)\}$ and define the \textit{productive subgraph} $G_{\delta}$ as $G_{\delta}=(V, \{(u,v)\in E: v \in N^*_u(\delta)\}$. For the single-token case, this graph signifies all the potential connections $(u,v)$ such that $u$ knows the token and $v$ doesn't or vice versa. Let $S(\delta)$ denote the subset of nodes that know the token and $n(\delta)=|S(\delta)|$. In the analysis, we will often want to refer to the smaller subset of nodes out of those who know the token and those who don't, as these nodes will limit how fast the token spreads. We denote this subset as $S^*(\delta)$ and define $n^*(\delta)=|S^*(\delta)|$.\\

The mobile telephone model captures the basic dynamics of the peer-to-peer libraries included in standard smartphone operating systems.
This abstraction, however, makes simplifying assumptions---namely, the assumption of synchronized rounds.
In this section we analyze the performance of simple random gossip processes in a more realistic version of the model that eliminates the synchronous round assumption.
In particular, we first define the  asynchronous mobile telephone model (aMTM), which describes an event-driven
peer-to-peer abstraction in which an adversarial scheduler controls the timing of key events in the execution.

An algorithm specified in the aMTM should be directly implementable on real hardware without the need to synchronize or simulate rounds.
This significantly closes the gap between theory and practice. 
With this in mind, after defining the aMTM, we specify and analyze a basic random gossip process strategy.
In this more realistic asynchronous model, different processes can be running at vasty different and changing speeds,
invalidating the clean round-based analysis from the previous section.
We will show, however, that even in this more difficult setting, 
random gossip processes can still be analyzed and shown to spread tokens with speed that increases with available connectivity.


\input{amtm}

\input{amtmAlgorithm}




==> dcoss 2019 -- full version/gossip.tex <==
\section{Random Gossip in the Mobile Telephone Model}
\label{sec:mtm}

Here we study a simple random gossip process in the mobile telephone model.
We begin by formalizing the model, the problem, and some graph theory preliminaries,
before continuing with the algorithm description and analysis.

\input{mtm}
\input{mtmAlgorithm}
%\input{sim}

==> dcoss 2019 -- full version/gossipProblem.tex <==
\subsection{The Gossip Problem}

% Motivate our study of the gossip problem in p2p networks
% Describe the gossip problem
% Give trivial algorithms that take O(kn) rounds and mention 2017 PODC results

==> dcoss 2019 -- full version/intro.tex <==
\section{Introduction} \label{sec:intro}

In this paper, we study random gossip processes in smartphone peer-to-peer networks.
We prove the best-known gossip bound in the standard synchronous model used to describe this setting,
and then establish new results  in a novel asynchronous variation of this model that more directly matches the real world behavior of smartphone networks.
Our results imply that  simple information spreading strategies work surprisingly well in this complicated but increasingly relevant environment.

In more detail, a random gossip process is a classical strategy for spreading messages through a peer-to-peer network.
It has the communicating nodes randomly select connection partners from their eligible neighbors,
and then once connected exchange useful information.\footnote{The main place where different random gossip processes vary is in their definition of ``eligible." 
What unites them is the same underlying approach of random connections to nearby nodes.}
As elaborated in Section~\ref{sec:related},
these random processes are well-studied in standard peer-to-peer models where they have been shown to spread information efficiently
despite their simplicity.


To date, however, little is known about these processes in the emerging setting of {\em smartphone} peer-to-peer networks,
in which nearby smartphone devices connect with direct radio links that do not require WiFi or cellular infrastructure.
As also elaborated in Section~\ref{sec:related}, 
both Android and iOS now provide support for these direct peer-to-peer
connections, enabling the possibility of smartphone apps that generate large peer-to-peer networks
that can be deployed, for example, when  
 infrastructure is unavailable (i.e., due to a disaster) or censored (i.e., due to government repression).
 This paper investigates whether the random gossip processes that have been shown to spread information well in other peer-to-peer
 settings will prove similarly useful in this intriguing new context.
 
\subsection{The Mobile Telephone Model (MTM)}
The \emph{mobile telephone model} (MTM), introduced by Ghaffari and Newport \cite{ghaffari:2016}, extends the well-studied 
\emph{telephone model} of wired peer-to-peer networks (e.g.,\cite{frieze1985shortest,telephone1,telephone2,telephone3,giakkoupis2011tight,chierichetti2010rumour,giakkoupis2012rumor,fountoulakis2010rumor,giakkoupis2014tight})
to better capture the dynamics of standard smartphone peer-to-peer libraries.
In recent years, 
several important peer-to-peer problems have been studied in
the MTM, including rumor spreading \cite{ghaffari:2016}, load balancing \cite{dinitz:2017}, leader election \cite{newport:2017}, and gossip \cite{newport:2017b}.


As we elaborate in Section~\ref{sec:mtm},
the mobile telephone model describes a peer-to-peer network topology with an undirected graph,
where the nodes correspond to the wireless devices, and an edge between two nodes indicates 
the corresponding devices are close enough to enable a direct device-to-device link.
Time proceeds in synchronous rounds.
At the beginning of each round,
each node can {\em advertise} a bounded amount of information to its neighbors in the topology.
At this point, each node can then decide to either send a connection {\em invitation} to a neighbor,
or instead receive these invitations, choosing at most one incoming invitation to accept, forming a connection.
Once connected, a pair of node can perform a bounded amount of communication before the round ends.
Each node is limited to participate in at most one connection per round.


\subsection{Gossip in the MTM}
The gossip problem assumes that $k$ out of the $n \geq k$ nodes start with a gossip message. The problem is solved once all nodes have learned all $k$ messages.
In the context of the MTM, we typically assume that at most $O(1)$ gossip messages can be transferred over a connection in a single round, and that advertisements are bounded 
to at most $O(\log{n})$ bits.

A natural random gossip process in this setting is the following: In each round, each node advertises a hash of its token set and flips a fair coin to decide whether to send or receive connection invitations. If a node $u$ decides to send, and it has at least one neighbor advertising a different hash (implying non-equal token sets), then it selects among these neighbors with uniform randomness to choose a single recipient of a connection invitation. If the invitation is accepted the two nodes exchange a constant number of tokens in their set difference.

It is straightforward to establish that with high probability in $n$ this process solves gossip in $O(nk)$ rounds.
The key insight is that in every round there is at least one potentially productive connection, and that there can be at most $O(nk)$ such connections before all nodes know all messages.
(See~\cite{newport:2017b} for the details of this analysis.)

In our previous work on gossip in the MTM~\cite{newport:2017b},
we explored the conditions under which you could improve on this crude $O(nk)$ bound.
We conjectured that a more sophisticated analysis could show that simple random processes improve on the $nk$ bound given sufficient graph connectivity,
but were unable to make such an analysis work.
Accordingly, in~\cite{newport:2017b} we turned our attention to a more complicated gossip algorithm called {\em crowded bin}.
Unlike the simple structure of random gossip processes, crowded bin requires non-trivial coordination among nodes,
having them run a distributed size estimation protocol (based on a balls-in-bins analysis) on $k$, and then using these estimates
to parametrize a distributed TDMA protocol that eventually enables $k$ independent token spreading processes to run in parallel.

In~\cite{newport:2017b}, we prove that crowded bin solves gossip in $O((k/\alpha)\log^5{n})$ rounds, with high probability in $n$,
 when run in a network topology with vertex expansion $\alpha$ (see below).
For all but the smallest values of $\alpha$ (i.e., least amounts of connectivity), this result is an improvement over the crude $O(nk)$ bound achieved by the random process.

A key open question from this previous work is whether or not it is possible to close the time complexity gap between the appealingly simple random gossip
processes and the more complicated machinations of crowded bin.
As we detail next, this is the question tackled in this paper.

\subsection{New Result \#1:  Improved Analysis for Gossip in the MTM}
In Section~\ref{sec:mtm}, 
we consider a variation of the simple random gossip process described above modified only slightly such that a node only considers a neighbor eligible if 
it advertises a different hash {\em and} it has not recently attempted a connection with that particular neighbor. We call this variation {\em random spread} gossip

By introducing a new analysis technique, we significantly improve on the straightforward $O(nk)$ bound for random gossip processes like random spread.
Indeed, we prove this process is actually slightly {\em more} efficient than the more complicated crowded bin algorithm
from~\cite{newport:2017b}, showing that with high probability in $n$, random spread requires only $O((k/\alpha)\log^4{n})$ rounds to spread all the messages
in a network with vertex expansion $\alpha$.

The primary advantage of random spread gossip is its simplicity. As with most random gossip processes,
its behavior is straightforward and easy to implement as compared
to existing solutions. 
A secondary advantage is that this algorithm works in the {\em ongoing} communication scenario in which new rumors
keep arriving in the system. Starting from any point in an execution, if there are $k$ rumors that are not yet fully disseminated,
they will reach all nodes in at most an additional $O((k/\alpha)\log^4{n})$ rounds, 
regardless of how many rumors have been previously spread.
%
The solution in~\cite{newport:2017b},
by contrast,
must be restarted for each collection of $k$ rumors,
and includes no mechanism for devices to discover that gossip has completed for the current collection.
Accordingly, this new result fully supersedes the best known existing results for gossip in the MTM under similar assumptions.\footnote{In~\cite{newport:2017b},
we also study gossip under other assumptions, like changing communication graphs and the lack of good hash functions.}

At the core of our analysis is a new data structure we call a {\em size band table} that tracks
the progress of the spreading rumors.
We use this table to support an amortized analysis of spreading that proves that
the stages in which rumors spread slowly are balanced out sufficiently by stages in which they spread quickly,
providing a reasonable average  rate. 


\subsection{New Result \#2: Gossiping in the Asynchronous MTM}
The mobile telephone model is a
high-level abstraction that captures the core dynamics of smartphone peer-to-peer communication,
but it does not exactly match the behavior of real smartphone networking libraries.
The core difference between theory and practice in this context is synchronization.
To support deep analysis, 
this abstract model (like many models used to study distributed graph algorithms)
synchronizes devices into well-defined rounds.
Real smartphones, by contrast, do not offer this synchronization.
%The time required for advertisements or connection invitations to propagate,
%and the rate at which communication occurs over accepted connections,
%might be bounded, but these bounds can vary between different deployments and are not known in advance to the algorithm.
It follows that algorithms developed in the mobile telephone model cannot be directly implemented on
real hardware.

With the goal of closing this gap,
in Section~\ref{sec:amtm}
we introduce the {\em asynchronous mobile telephone model} (aMTM),
a variation of the MTM that removes the synchronous round assumption,
allowing nodes and communication to operate at different speeds.
The main advantage of the aMTM, is that algorithms specified and analyzed
in the aMTM can be
directly implemented using existing smartphone peer-to-peer libraries.
The main disadvantage is that the introduction of asynchrony complicates analysis.

In Section~\ref{sec:amtm},
we first study the question of whether simple random gossip processes even still converge in a setting
where nodes and messages can operate at different speeds controlled by an adversary. 
We answer this question positively by proving that a simple random gossip process solves gossip in $O(nk\delta_{max})$
time, where $\delta_{max}$ is an upper bound on the maximum time certain key steps can occur
(as is standard, we assume $\delta_{max}$ is determined by an adversary, can change between executions, and is unknown to
the algorithm).

 We then tackle the question of whether it is still possible to show
 that the time complexity of
  information spreading improves with vertex expansion in an asynchronous setting.
  The corresponding analyses in the synchronous MTM,
  which treats nodes as implicitly running an approximate maximum matching algorithm between nodes that know a certain token and those that do not,
   depend heavily on the synchronization of node behavior.
   
   We introduce a novel analysis technique,
 in which we show that the probabilistic connection behavior in the aMTM over time sufficiently approximates
 synchronized behavior to allow our more abstract graph theory results to apply.
 %
 In particular, we prove that for $k=1$, the single message spreads in at most $O(\sqrt{(n/\alpha)}\cdot \log^2{n\alpha} \cdot \delta_{max})$ time.
 This result falls somewhere between our previous $O(n \delta_{max})$ result for gossip with $k=1$ in the aMTM,
 and the bound of $O(\text{polylog}(n)/\alpha)$  rounds possible in the synchronous MTM for $k=1$.
 The remaining gap with the synchronous results seems due
  the ability of synchronous algorithms to keep a history of recent connection attempts (crucial to the underlying matching analysis),
 whereas in the asynchronous model such histories might be meaningless if some nodes are making connections attempts much faster than others.
 
We argue that our introduction of the aMTM, as well as a powerful set of tools for analyzing information spreading in this setting,
provides an important foundation for the future study of communication processes in realistic smartphone peer-to-peer models.
 
 \iffalse



\subsection{OLD}
In this paper, we explore random spread gossip algorithms designed for peer-to-peer communication protocols available in modern smartphones. While gossip is a well-studied problem in distributed systems research, existing solutions are difficult to implement on existing devices. One issue is that classic abstractions do not accurately capture the interfaces provided by these libraries. Another obstacle is the difficulty of designing algorithms that provide strong performance guarantees yet are simple enough to implement easily. This paper approaches both of these challenges by extending known abstractions for this setting to better represent communication in these peer-to-peer networks and introducing simple algorithms that achieve the best known performance for these models.

\subsection{Motivation}

The ubiquity of smartphones is increasingly matched by the availability of peer-to-peer communications libraries on these devices. Libraries such as Bluetooth \cite{gomez2012overview}, Wi-Fi Direct \cite{camps2013device}, and Apple's Multipeer Connectivity Framework (MPC) \cite{multipeer} allow devices to leverage one-hop radio links to form large-scale mesh networks that enable communication in the absence of cellular or Wi-Fi infrastructure. The implications of these networks are widespread and signficant. Recent research, for example, uses smartphone peer-to-peer networks to 
support disaster response~\cite{suzuki2012soscast,reina2015survey,lu2016networking}, 
circumvent censorship~\cite{firechat}, extend internet access~\cite{aloi2014spontaneous,oghostpot},
support local multiplayer gaming~\cite{mark2015peer} and improve classroom interaction~\cite{holzer2016padoc}.
This networking platform is particularly exciting as smartphones are already widely used and supported,
 minimizing one of the major obstacles to ad hoc network research:
the difficulty of developing and deploying custom technology.

While these networks offer an exciting opportunity for a new wave of smartphone applications, it is important that we rely on more than standard software development practices to create them. By applying results from the extensive field of distrubted algorithms theory, we can unlock new strategies for meeting the many networking challenges these emerging applications are likely to encounter. However, the restrictive interfaces of these libraries prevent the direct usage of classic implementations of the necessary networking primitives. For example, not only are devices restricted to a local view of the network (ie. nodes only have knowledge of their neighbors), processes can only engage in a constant number of connections at a time. This is a significant weakness compared to more typical network settings where processes may freely communicate with their entire neighborhood, but modern peer-to-peer libraries offer a powerful tool for mitigating this limitation. Namely, they allow a device to broadcast a small amount of information, called an \emph{advertisement}, to all its neighbors before attempting to form a connection. Clearly, substantial new theoretical work is required to apply rigorous analysis to this new scenario.

\subsection{The Mobile Telephone Model}

One approach to formalizing the algorithmic analysis of this setting is to define an abstraction that captures its core properties, and then in the context of this abstraction apply algorithm theory to identify and rigorously analyze local communication strategies that generate the desired global behavior. The \emph{mobile telephone model}, introduced by Ghaffari and Newport \cite{ghaffari:2016}, is an example of this method. This abstraction, described fully in section \ref{sec:mtm}, extends the well-studied \emph{telephone model} to better capture the unique properties of smartphone peer-to-peer networks described above. In this model, a network of wireless devices is represented as an undirected graph with each device corresponding to a node in the graph. An edge between two nodes represents the ability of these nodes to connect to each other, often indicating that the corresponding devices are close enough together. Time in this abstraction proceeds in synchronous rounds divided into two phases, \emph{scan} and \emph{connect}. In the scan phase, devices set a bounded amount of information called an \emph{advertisement} or \emph{tag} that is broadcast to its neighbors in the topology. In the subsequent connection phase, devices choose to either send a connection invitation to a neighbor, or receive invitations from its neighbors and accept at most one. Once an invitation is accepted, a connection is formed between two nodes, enabling them to communicate a bounded amount of information before the end of the round. The restriction that each node may only engage in a single connection per round and the ability to broadcast advertisements before these connections are formed are the key properties of this model that make it ideal for studying smarphone peer-to-peer networks.

In recent work, many algorithms have been developed for problems in this setting; including rumor spreading \cite{ghaffari:2016}, load balancing \cite{dinitz:2017}, leader election \cite{newport:2017}, and gossip \cite{newport:2017b}. Though these problems have been studied in other peer-to-peer models,novel techniques were required to achieve useful boundsunder the unique constraints of the smartphone peer-to-peersetting. These results, therefore, provide useful insights into implementing peer-to-peer functionality on smartphones.

\subsection{Random Spread Gossip}

The gossip problem assumes that there are $k$ pieces of information called \emph{rumors} in the network, for some parameter $k\geq 1$, that must be spread. The problem is solved once all $n$ devices in the network receive all $k$ rumors. Gossip is considered to be a key primitive in peer-to-peer settings (c.f., \cite{shah:2009}), justifying its study in the emerging smartphone peer-to-peer scenario.

In the context of \emph{scan}-and-\emph{connect} abstractions such as the mobile telephone, rumors are assumed to be large enough that they can only be transmitted through an established connection. Furthermore, an intuitive strategy for choosing these connections is called \emph{random spread gossip}, in which which nodes choose one of their eligible neighbors uniformly at random to connect to. The primary advantage of random spread gossip is its simplicity. Its behavior is straightforward and easy to implement as compared to existing solutions.

\subsection{This Paper}

In this paper, we address two substantial challenges to implementing gossip algorithms on these peer-to-peer networks by refining current abstractions and analyzing the performance of random spread gossip algorithms on these models.

\paragraph{Contribution \#1. Random Spread Gossip in the Mobile Telephone Model} The best known gossip algorithm for the mobile telephone model solves the problem in $\bigO{(k/\alpha)\log^5{n}}$ rounds (with high probability in $n$)~\cite{newport:2017b}, where $\alpha$ describes the vertex expansion of the underlying network topology (see Section~\ref{sec:model:vertex}). A drawback of this existing algorithm is its complexity. It requires devices to run multiple instances of a TDMA-style rumor spreading strategy in parallel, each parameterized to a different guess at $k$. A randomized balls-in-bins process is used to help devices eventually converge on a reasonable estimate of $k$, enabling faster progress for the rumors.

In Section~\ref{sec:alg}, we describe a simpler algorithm we call random spread gossip. A secondary advantage is that this algorithm works in the ongoing communication scenario in which new rumors keep arriving in the system. Starting from any point in an execution, if there are $k$ rumors that are not yet fully disseminated, they will reach all nodes in at most an additional $\bigO{(k/\alpha)\log^4{n}}$ rounds, regardless of how many rumors have been previously spread. The solution in~\cite{newport:2017b}, by contrast, must be restarted for each collection of $k$ rumors, and includes no mechanism for devices to discover that gossip has completed for the current collection.

At the core of our analysis is a new data structure we call a {\em size band table} that tracks the progress of the spreading rumors. We use this table to support an amortized analysis of spreading that proves that the stages in which rumors spread slowly are balanced out sufficiently by stages in they spread quickly to guarantee a reasonable average dissemination rate. 

\paragraph{Contribution \#2. Model Simulation} The mobile telephone model is a high-level abstraction that captures the core dynamics of smartphone peer-to-peer communication, but does not exactly match the behavior of real smartphones. The core difference is synchronization. To support deep analysis, this abstract model (like many models used to study distributed graph algorithms) synchronizes devices into well-defined rounds. Real smartphones, by contrast, do not offer this synchronization. It follows that algorithms developed in the mobile telephone model cannot be directly implemented on
real hardware.

With the goal of closing this gap, in Section~\ref{sec:sim} we turn our attention to Apple's Multipeer Connectivity Framework~\cite{multipeer}: the peer-to-peer library included in every iOS release since version 7.  We focus on iOS because its peer-to-peer support is arguably more developed than what is currently available on the Android platform. Among other advantages, it hides the end user from the underlying communication protocols---e.g., WiFi, Bluetooth---providing a generic interface for advertising, scanning for advertisements, and attempting to setup connections.

We describe a new algorithm called MTM sim that {\em simulates} the mobile telephone model using the Multipeer Connectivity Framework. Roughly speaking, this simulator carefully partitions each simulated round into several stages, and uses the multipeer advertisements to keep nearby devices sufficiently synchronized as they pass through the stages. We apply a result from the classical synchronizer literature of the 1980s to establish that the  average time required to simulate a mobile telephone model round is within a constant factor of the time required for discovery and connection on the underlying peer-to-peer framework.

\paragraph{Contribution \#3. Random Spread Gossip in the Asynchronous Mobile Telephone Model} The synchronization strategy presented in section \ref{sec:sim}, while adding only a constant factor to the time complexity of the random spread gossip algorithm, adds substantial overhead. Since this overhead is a consequence of implementing mobile telephone model algorithms on real devices, we explore instead an extension of the MTM that we introduce in this paper, the \emph{asynchronous mobile telephone model}. Once again using the Multipeer Connectivity Framework API as a template, we design a model that consists of function calls available to the algorithm and callback hooks that the model can use to respond. Our interface, like the MPC, abstracts all details of the underlying communication primitives. 

Our final contribution is the introduction of a second random spread gossip algorithm for the asynchronous mobile telephone model, simply called \emph{asynchronous random spread gossip}. This algorithm is the natural progression from the synchrous random spread gossip algorithm in section \ref{sec:alg} for the asynchronous setting. This algorithm, as in the synchronous version, supports ongoing communication. Unlike in the synchronous version, however, this algorithm is directly applicable to the smartphone setting and provices fault tolerance guarantees. We analyze this algorithm to show that its performance scales well with the vertex expansion of the network and therefore is efficient for well-connected graphs.

\fi



==> dcoss 2019 -- full version/mtm.tex <==
\subsection{The Mobile Telephone Model}
\label{sec:mtm}

%\label{sec:mtm}
%
The mobile telelphone model describes a smartphone peer-to-peer network topology as an undirected connected graph 
$G=(V,E)$. A computational process (called a {\em node} in the following) is assigned to each vertex in $V$.
%Let $n=|V|$  indicates the network size.
The edges in $E$ describe which node pairs are within communication range.
In the following, we use $u\in V$ to indicate both the vertex in the topology graph as well
as the computational process (node) assigned to that vertex.
We use $n=|V|$ to indicate the network size. 


Executions proceed in synchronous rounds labeled $1,2,...$,
and we assume all nodes start during round $1$.
%The standard assumption is that all nodes start during the same round.
%We will later address a straightforward strategy to synchronize the round numbers in a setting
%where nodes join the network a different times.
%
At the beginning of each round,
each node $u\in V$ selects an {\em advertisement} to broadcast to its neighbors $N(u)$ in $G$.
This advertisement is a bit string containing no more than $O(\log{n} + \ell_h)$ bits,
where $\ell_h$ is the digest length of a standard hash function parameterized to obtain the 
desired collision resistance guarantees.
After broadcasting its advertisement,
node $u$ then receives the advertisements broadcast by its neighbors in $G$ for this round.
%\footnote{In earlier studies of the mobile telephone model,
%we described the tag length with a parameter $b$ and considered smaller bounds such as $b=1$ and $b=\log\log{n}$.
%As described in our discussion of the practical Mobile Telephone Model,
% subsequent experimentation with real smartphone peer-to-peer standards revealed that the advertisement tags are actually quite large,
 %and both $\log{n}$ and $\ell_h$ are conservative bounds for the number of bytes allowed for these advertisements in real systems.}

At this point, $u$ decides to either {send} a {\em connection invitation}
to a neighbor, or passively receive these invitations.
If $u$ decides to receive, and at least one connection invitation arrives at $u$, 
then node $u$ can select at most one such incoming invitation to {\em accept}, forming a connection
between $u$ and the node $v$ that sent the accepted invitation.
Once $u$ and $v$ are connected,
they can perform a bounded amount of reliable interactive communication before the round ends,
where the magnitude of this bound is specified as a parameter of the problem studied.
%
%
Notice that the model does not guarantee to deliver $u$ all invitations sent to $u$ by its neighbors.
It instead only guarantees that if at least one neighbor of $u$ sends an invitation,
then $u$ will receive a non-empty subset (selected arbitrarily)
of these invitations before 
it must make its choice about acceptance. 

If $u$ instead chooses to send a connection invitation to a neighbor $v$,
there are two outcomes. If $v$ accepts $u$'s invitation,
a connection is formed as described above.
Otherwise, $u$'s invitation is implicitly rejected.


\iffalse

\subsection{The Practical Mobile Telephone Model}
\label{sec:pmtm}

The practical mobile telephone model (pMTM) more directly describes
the peer-to-peer interface provided by iOS devices than the MTM. While it describes the same graph topology as the MTM, its purpose is to better capture the asynchronous setting of realistic smartphone networks by allowing nodes to proceed in rounds independently of other nodes. In this model, nodes can make particular function calls but must also react to events initiated by the model at any time. They can also implement timers to wait a certain amount of time before continuing execution but cannot use timers in an attempt to synchronize with other nodes. The model assumes that $r_{min}$, $r_{max}$, and $b_{max}$ are known to the algorithm while the definitions of $\delta_{a}$, $\delta_{i}$, $\delta_c$, and $\delta_d$ are not known in advance and can change from execution to execution.

\bigskip

\noindent Any node executing an algorithm using the pMTM has access to the following functions:

\begin{itemize}

	\item $SetAdv(tag)$: changes the node's advertisement tag to $tag$, includes the decision to \emph{send} or \emph{receive} connection proposals
	\item $Invite(user,info)$: sends a connection invitation to a single $receiver$ neighbor specified by $user$ along with context information $info$ (the latter
	detailing, for example, the purpose for the invitation, etc\ldots). This is called by a $sender$ node after receiving at least one new advertisement from a neighboring $receiver$ through the $AdvTableUpdate(user,tag)$ event
	\item $AcceptInvite(user_{inviting},info)$: accepts a single invitation with context $info$ received from $user_{inviting}$ after the $ReceiveInvite(user_{inviting},info)$ event and initiates a connection attempt with user
	\item $RejectInvite(user_{inviting},info)$: rejects an invitation with context $info$ from neighbor $user_{inviting}$ after the $ReceiveInvite(user_{inviting},info)$ event
	\item $SendData(data, user_{connected})$: begins sending data resource $data$ to a connected neighbor $user_{connected}$ after a connection is formed, identified by the $Connected(user_{connected})$ event
	\item $Disconnect(user)$: terminates the connection formed with neighbor $user$, can only be called after the $Connected(user_{connected})$ event
	\end{itemize}

\noindent Nodes executing an algorithm using the pMTM must implement the following callback functions corresponding to a number of events that may be triggered by the model:
\begin{itemize}
\item $AdvTableUpdate(user,tag)$: an update of the neighbor $user$'s advertisement tag to $tag$ is detected
\item $ReceiveInvite(user_{inviting}, info)$: a connection attempt from $user_{inviting}$ with context $info$ is received. The algorithm can then call $AcceptInvite(user_{inviting})$ or $RejectInvite(user_{inviting})$ to respond.
\item $InviteAccepted(user_{invited}, info)$: node $user_{inviting}$ accepted a connection proposal from this node with context $info$
\item $InviteRejected(user_{invited}, info)$: node $user_{inviting}$ rejected a connection proposal from this node with context $info$
	\item $Connected(user_{connected})$: a connection is formed with a neighboring process $user_{connected}$ after either $user_{connected}$ accepted a connection invitation from this process or this process accepted an invitation from $user_{connected}$
	\item $ReceivedData(user_{connected}, data)$: finished receiving some data resource $data$ from $user_{connected}$
	\item $Disconnected(user)$: the connection with a neighbor $user$ was terminated
\end{itemize}

\noindent The model provides the following guarantees:

\begin{itemize}

\item If a process $u$ calls $SetAdv(t)$ for some tag $t$, all neighboring processes will call $AdvTableUpdate(u,t)$ within at most time $\delta_a$ as long as $u$ doesn't call $SetAdv(t^\prime)$ for some new tag $t^\prime$ during this interval.
\item If a process $u$ calls $Invite(v,i)$ for some neighboring process $v$ and context $i$, $v$ will call $ReceiveInvite(u, i)$ within at most time $\delta_i$. If $v$ calls $AcceptInvite(u,i)$, $u$ will call $InviteAccepted(v,i)$ within at most time $\delta_i$ as well.
\item If a process $u$ calls $InviteAccepted(v,i)$ for some neighboring process $v$ and context $i$, $u$ will call $Connected(v)$ and $v$ will call $Connected(u)$ within at most time $\delta_c$.

\item Once a connection is formed between two nodes $u$ and $v$, if $u$ calls $sendData(d,v)$ for some resource $d$ with name $n$, within some worst-case time bound $v$ will call $ReceivingData(n, u)$ and subsequently $ReceivedData(n, u, d)$ dictated by a bit rate in the range of bit rates $[r_{min}, r_{max}]$.
\item If a process $u$ calls $Disconnect(v)$ for some neighboring process $v$, $u$ will call $Disconnected(v)$ and $v$ will call $Disconnected(u)$ within at most time $\delta_d$.
\item All advertisement tags specified by the parameter $tag$ and context information specified by the parameter $info$ have a maximum number of bits $b_{max}$.
\end{itemize}

\fi

\subsection{The Gossip Problem}
\label{sec:model:gossip}
The gossip problem is parameterized with a token count $k>0$.
It assumes $k$ unique {\em tokens} are distributed to nodes at the beginning of the execution.
The problem is solved once all nodes have received all $k$ tokens.
We treat the tokens as black boxes objects that are large compared to the advertisements.
With this in mind, we assume the only ways 
for a node $u$ to learn token $t$ are: (1) $u$ starts with token $t$; or (2) a node $v$ that previously learned $t$
sends the token to $u$ during a round in which $v$ and $u$ are connected.

We assume that at most a constant number of tokens can be sent over a given connection.
Notice that this restriction enforces a trivial $\Omega(k)$ round lower bound for the problem.



\subsection{Vertex Expansion}
\label{sec:model:vertex}

%\label{sec:vertex}
Some network topologies are more suitable for information dissemination than others.
In a clique, for example, a message can spread quickly through epidemic replication,
while spreading a message from one endpoint of a line to another is necessarily slow.
With this in mind,
the time complexity of
information dissemination algorithms are often expressed with respect to graph connectivity
metrics such as {\em vertex expansion} or {\em graph conductance}.
In this way, an algorithm's performance can be proved to improve along with available connectivity.

In this paper, 
as in  previous studies of algorithms in the mobile telephone model~\cite{ghaffari:2016,dinitz:2017,newport:2017,newport:2017b},
we express our results with respect to vertex expansion (see~\cite{ghaffari:2016} for an extended discussion
of why this metric is more appropriate than conductance in our setting).
Here we define this metric and establish a useful related property.

For fixed undirected connected graph $G=(V,E)$,
and a given $S \subseteq V$, we define the {\em boundary} of $S$, indicated $\partial S$, as follows:
 $\partial S = \{ v\in V \setminus S : N(v) \cap S \neq \emptyset\}$: that is, $\partial S$ is the set
 of nodes not in $S$ that are directly connected to $S$ by an edge in $E$.
 We define $\alpha(S) = |\partial S|/|S|$.
We define the {\em vertex expansion} $\alpha$ of a given graph $G = (V,E)$
 as follows:
 
 \[  \alpha = \min_{S \subset V, 0 < |S| \leq n/2} \alpha(S). \]
 
 \noindent Notice that despite the possibility of $\alpha(S) >1$ for some $S$, we always have $\alpha \leq 1$.
In more detail, this parameter ranges from $2/n$ for poorly connected graphs (e.g., a line)
to values as large as $1$ for well-connected graphs (e.g., a clique).
Larger values indicate more potential for fast information dissemination.



%\paragraph{Connecting Expansion to Independence Number.}
The mobile telephone model requires the set of pairwise connections in a given round to form a matching
in the topology graph $G=(V,E)$.
The induces a connection between
maximum matchings and the maximum amount of potential communication in a given round.
Here we adapt a useful result from~\cite{ghaffari:2016} that formalizes
the relationship between vertex expansion and these matchings as defined with respect
to given partition.

In more detail, 
for a given graph $G=(V,E)$ and node subset $S\subset V$,
we define $B(S)$ to be the bipartite graph with bipartitions $(S,V \setminus S)$,
and the edge set $E_S = \{ (u,v): (u,v) \in E$, $u\in S$, and $v\in V \setminus S\}$.
 Recall that the {\em edge independence number} of a graph $H$,
denoted $\nu(H)$, describes the size of a maximum matching on $H$.
For a given $S$, therefore, $\nu(B(S))$ describes the maximum number 
of concurrent connections that a network can support in the mobile telephone model between nodes in $S$
and nodes outside of $S$.  This property follows from the restriction in this model that each node can participate
in at most one connection per round. 

The following result notes that the vertex expansion does a good job of approximating the size
of the maximum matching across any partition:

 \begin{lemma}[from~\cite{ghaffari:2016}]
 Fix a graph $G=(V,E)$ with $|V| = n$ with vertex expansion $\alpha$.
Let $\gamma = \min_{S\subset V, |S| \leq n/2}\{ \nu(B(S))/|S|  \}$.
It follows that $\gamma \geq \alpha/4$.
\label{lem:msize}
\end{lemma}



%\paragraph{Discussion.}
%\note{Need some discussion. Add citations to other papers that use vertex expansion.
%Note that $\log{n}/\alpha$ lower bound. Point to our paper from 2016 to establish that graph conductance---which is often used
%in other peer-to-peer models---is not a good parameter in mobile telephone model. It is easy to show that there exists
%graphs with good conductance but where efficient information dissemination is impossible if connections are a matching in each round (i.e., give star example).}


%We measure the performance of a given gossip algorithm by the number of rounds required for
%it to solve the problem (disseminate the $k$ tokens to all $n$ nodes) with a given probability.
%We will typically express these time bounds as a combingation of the network size, token count,
%and relevant graph parameter capturing the connectedness of $G$ (e.g., vertex expansion).


==> dcoss 2019 -- full version/mtmAlgorithm.tex <==

\subsection{The Random Spread Gossip Algorithm}
\label{sec:alg}

%We begin by describing the random spread gossip algorithm.
%We then analyze its time complexity.
 
%\subsection{Algorithm Description.}
We formalize our random spread gossip algorithm with the pseudocode labeled Algorithm~1.
Here we summarize its behavior.

The basic idea of the algorithm is that in each round, each node advertises a hash of their token set.
Nodes then attempt to connect only to neighbors that advertised a different hash, 
indicating their token sets are different. 
When two nodes connect,
they can transfer a constant number of tokens in the non-empty set difference
of their respective token sets.

As detailed in the pseudocode, the random spread algorithm implements the above strategy combined with some minor additional structure
that supports the analysis. 
In particular, nodes partition rounds into {\em phases} of length $\lceil \log{N} \rceil$, where $N > 1$ is an upper bound on the maximum
degree $\Delta$ in the network topology.
Instead of each node deciding whether to send or receive connection invitations at the beginning of {\em each round},
they make this decision at the beginning of {\em each phase}, and then preserve this decision throughout the phase (this is captured in the pseudocode
with the $status$ flag that is randomly set every $\lceil \log{N} \rceil$ rounds).
Each receiver node also advertises whether or not it has been involved in a connection already during the current phase
(as captured with the $done$ flag).
A sender node will only consider neighbors that advertise a different hash, are receivers in the current phase,
{\em and} have not yet been involved in a connection during the phase.




%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}

% -------------------------------------------------------
\begin{algorithmic}
\State
\State \underline{Initialization:}  
\State $N \gets$ upper bound on maximum degree in topology
\State $T \gets$ initial tokens (if any) known by $u$
\State $H$ is a hash function
\State
\State \underline{For each round $r$:}
\State
\If{$r$ mod $\lceil \log{N} \rceil$ = 1}
	\State $status \gets$ random bit (1=sender; 0=receiver)
	\State $done \gets 0$
\EndIf
\State
\State {\tt Advertise}$(\langle status, done, H(T,r), u \rangle)$ 
\State $A \gets$ {\tt RecvAdvertisements}$()$
\State
\State $A' \gets \{ v\mid \langle 0,0,h,v \rangle \in A, h \neq H(T,r)\}$
\If{$status=1$ {\bf and} $|A'| > 0$} 
	\State $v \gets$ node selected with uniform randomness from $A'$
	\State {\em (Attempt to connect with $v$. If successful, exchange a token in set difference.)}
	%\State {\bf SendConnectionProposal}$(v)$
	%\State (If $v$ accepts then exchange a token in the set difference and set $done \gets 1$)
\ElsIf{$status=0$} 
	\State {\em (If receive connection proposal(s): accept one, exchange token in the set difference,  set $done \gets 1$.)}
\EndIf
\end{algorithmic}
% -------------------------------------------------------

\label{alg:1}
\caption{Random spread gossip (for node $u$).}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%

\subsection{Analysis of Random Spread Gossip}
Our goal is to prove the following result about the performance of random spread gossip:

\begin{theorem}
With high probability, 
the random spread gossip algorithm solves the gossip problem 
in $O((k/\alpha)\log^2{n}\log{N}\log{\Delta})$ rounds, when executed with $k>0$ initial tokens and degree bound $N\geq \Delta$,
 in a network topology graph of size $n$, maximum degree $\Delta$, and vertex expansion $\alpha$.
\label{thm:main}
\end{theorem}




We begin by establishing some preliminary notations and assumptions before continuing to
the main proof argument.





\paragraph{Notation}
For a fixed execution, 
let $Q$ be the non-empty set of $k$ tokens that the algorithm must spread.
For each round $r>0$ and node $u\in V$,
let $T_u(r)$ be the tokens (if any) ``known" by $u$ at the start of round $r$
(that is, the tokens that $u$ starts with as well as every token it received through a connection in rounds $1$ to $r-1$).

For each $t\in Q$, and round $r>0$, let $S_t(r) = \{  v: t\in T_v(r)\}$ be the nodes that know token $t$ at the start of round $r$.
Let $n_t(r) = |S_t(r)|$ be the number of nodes that know token $t$ iat the beginning of this round,
and let $n^*_t(r) = \min\{ n_t(r), n-n_t(r)   \}$.



%
Finally, let  %$q^*(r) = \max_{t\in Q}\{n^*_t(r)\}$ be the maximum of these values over all $k$ tokens,
 $t^*(r)=\text{argmax}_{t\in Q}\{n^*_t(r)\}$ be a token $t$ with the maximum $n^*_t(r)$ value in this round (breaking ties arbitrarily).
 According to Lemma~\ref{lem:msize},
which connects vertex expansion to matchings,
there is a matching between nodes in $S_{t^*(r)}(r)$ and $V\setminus S_{t^*(r)}(r)$ of
size at least $(\alpha/4)\cdot n^*_{t^*(r)} (r)$.
Token $t^*(r)$, in other words,
has the largest guaranteed potential to spread in round $r$ among all tokens.\footnote{To be slightly more precise,
$(\alpha/4)\cdot n^*_{t^*(r)}(r)$ is a lower bound on the size of the matching across the cut
defined by $t^*(r)$, so $t^*(r)$ is the token with the largest lower bound guarantee on the size of its matching.}
Accordingly, in the analysis that follows,
we will focus on this token in each phase to help lower bound the amount of spreading we hope to achieve.

 
 \paragraph{Productive Connections and Hash Collisions}
 In the following, we say a given pairwise connection between nodes $u$ and $v$  in some round $r$ is {\em productive} if 
 $T_u(r) \neq T_v(r)$. That is, at least one of these two nodes learns a new token during the connection.
 By the definition of our algorithm, 
 if $u$ and $v$ connect in round $r$,
 then it must be the case that $H(T_u(r),r) \neq H(T_v(r),r)$,
 where $H$ is the hash function used by the random spread gossip algorithm.
 This implies $T_u(r) \neq T_v(r)$---indicating that every connection created by our algorithm is productive.
 
 On the other hand, it is possible for some $u$, $v$, and $r$ that even though $T_u(r) \neq T_v(r)$,
 $H(T_u(r),r) = H(T_v(r),r)$ due to a hash collision.
 For the sake of clarity, in the analysis that follows we assume that no hash collisions occur in the analyzed execution.
 Given the execution length is polynomial in the network size $n$,
 and there are at most $n$ different token sets hashed in each round,
 for standard parameters the probability of a collision among this set would be extremely small, supporting our assumption.
 
 We emphasize, however, that even if a small number of collisions {\em do} occur, 
 their impact is minimal on the performance of random spread gossip.
 The worst outcome of a hash collision in a given round
 is that during that single round a potentially productive connection is not observed to be productive and therefore 
 temporarily ignored. As will be made clear in the analysis that follows, the impact of this event is nominal.
 Indeed,
 even if we assumed that up to a constant fraction of the hashes in every round generated collisions---an extremely unlikely event for all but the weakest hash function parameters---the algorithm's worst case time complexity would decrease
 by at most a constant factor.
  
\paragraph{Matching Phases}
Recall that our algorithm partitions rounds into {\em phases} of length $\lceil \log{N}\rceil$.
For each phase $i>0$,
let $r_i = \lceil \log{N} \rceil\cdot (i-1) + 1$ be the first round of that phase.
Fix some arbitrary phase $i$
and consider token $t=t^*(r_i)$,
which, as argued above, is the token with the largest guaranteed potential to spread
in round $r_i$.
Our goal in this part of the analysis is to prove that with constant probability,
our algorithm will create enough productive connections during this phase to well-approximate
this potential.
This alone is not enough to prove our algorithm terminates efficiently,
as in some phases, it might be the case that {\em no} token has a large potential to spread.
The next part of our argument will tackle this challenge by proving that over a sufficient number
of phases the aggregate amount of progress must be large.

We begin by
establishing the notion of a {\em productive subgraph}:

\begin{definition}
At the beginning of any round $r>0$, we define the {\em productive subgraph} of the network
topology $G=(V,E)$ for $r$ as: $G_r = (V,E_r)$, where
$E_r = \{ \{u,v\}\mid \{u,v\}\in E, T_u(r) \neq T_v(r),u.status(r) \neq v.status(r)\}$,
and for each $w\in V$, $w.status(r)$ indicates the value of the node $w$'s status bit 
for the phase containing round $r$. 
\end{definition}

That is, the productive subgraph for round $r$ is the subgraph of $G$ that contains
only edges where the endpoints: (1) have different token set; and (2) have
different statuses (one is a sender during this phase and one is a receiver).
This subgraph contains every possible connection for a given round of our gossip algorithm
(we ignore $done$ flags because, as will soon be made clear,
we consider these graphs defined only for the first round of phases, a point at
which all $done$ flags are reset to $0$).
Accordingly, a maximum matching on this subgraph upper bounds the maximum number
of concurrent connections possible in a round.

We begin by lower bounding the size of the maximum matching in a productive subgraph at the beginning of a given phase $i$
using the token $t=t^*(r_i)$. Recall that $n^*_t(r_i)$ is the number of nodes that know token 
$t$ at the beginning of $r$, if less than half know the token, and otherwise indicates
the number of nodes that do not know $t$.

\begin{lemma}
Fix some phase $i$.
Let $t= t^*(r_i)$.
Let $G_{r_i}$ be the productive subgraph for round $r_i$,
 $M_{i}$ be a maximum matching on $G_{r_i}$, and $m_i = |M_{i}|$.
With constant probability (defined over the $status$ assignments):
$m_i \geq (\alpha/16)n^*_t(r_i)$. 
\label{lem:prod}
\end{lemma}
\begin{proof}
Fix some phase $i$.
We define $G'_{r_i}$ to be the {\em potentially productive} subgraph for round $r_i$,
where {\em potentially productive} is defined the same as {\em productive} except
we {\em omit} the requirement that endpoints of edges in the graph have different $status$ values.
 Let $M'$ be a maximum matching on $G'_{r_i}$ and $m' = |M'|$.
 We will reason about $m'$ as an intermediate step toward bounding the size of the actual productive subgraph
 for this round.
 
 
Let $t=t^*(r_i)$.
Consider the cut between nodes that know $t$, and nodes that do not,
 at the beginning of this phase.
 %; i.e.,
%the cut defined by 
% $Q = V \setminus S_t(r_i)$.
By Lemma~\ref{lem:msize}, 
there is a matching across this cut of size at least $(\alpha/4)n^*_t(r_i)$.
By definition, for all edges across this cut, their endpoints have different
token sets at the beginning of round $r_i$, 
therefore they are all candidates to be included in $M'$,
implying that $m' \geq  (\alpha/4)n^*_t(r_i)$.


Our next step is to consider the random assignment of sender and receiver status to nodes in $M'$
at the beginning of phase $i$.
For an edge in $M'$ to be included in a matching on the productive subgraph $G_{r_i}$,
 it must be the case that 
one endpoint chooses to be a receiver while the other chooses to be a sender.
We call such an edge {\em good}.
For any particular edge $e \in M'$,
this occurs with probability $1/2$. 

For each such $e\in M'$, 
 let $X_e$ be the random indicator that evaluates to $1$ if $e$ is good, and evaluates to $0$ otherwise.
 Let $Y=\sum_{e\in M'} X_e$ be the number of good edges for this phase.
By our above probability calculation, we know:

\[ E[Y] = E\left[ \sum_{e\in M'} X_e \right] = \sum_{e\in M'} E[X_e] = m'/2. \]

Because $M'$ is a matching, these indicator variables are independent. 
This allows us to concentrate on the mean.
In particular,
we will apply the following multiplicative Chernoff Bound, 
defined for $\mu = E[Y]$ and any $0\leq \delta \leq 1$:

\[ \Pr(Y \leq (1-\delta)\mu) \leq e^{- \frac{\delta^2\mu}{2}}, \]

\noindent with $\delta=1/2$, to establish that the probability that $Y \leq m'/4$ is upper bounded by:

\[  e^{- \frac{\mu}{8}} = e^{- m'/16   } < .94. \]

It follows that $Y$ is less than or equal to  $m'/4$, which is itself greater
than or equal to $(\alpha/16)n^*_t(r_i)$
with a probability upper bounded by a constant---as required.\footnote{Clearly,
 the specific worst failure bound of $0.06$ is loose (in the worst case, where $m_i=1$, for example,
we can directly calculate that $Y=m_i$ with probability $1/2$). We are not,
however, attempting to optimize constants in this analysis,
so any constant bound is sufficient
for our purposes.}
\end{proof}

We now turn our attention to our gossip algorithm's ability to take advantage
of the potential productive connections captured by the productive subgraph defined
at the beginning of the phase. 
To do so, we first adapt a useful result on rumor spreading from~\cite{ghaffari:2016}
to the behavior of our gossip algorithm.
Notice that it is the proof of the below adapted lemma that requires
the use of the $done$ flag in our algorithm.

\begin{lemma}[adapted from Theorem 7.2 in~\cite{ghaffari:2016}]
Fix a phase $i$.
Let $G'$ be a subgraph of the productive subgraph $G_{r_i}$ that satisfies the following:
\begin{enumerate}
\item there is a matching of size $m$ in $G'$;
\item the set $L$ of nodes in $G'$ with sender status is of size $m$; and
\item for each node $u\in L$, every neighbor of $u$ in $G_{r_i}$ is in $G'$. 
\end{enumerate}
With constant probability (defined over the random neighbor choices), 
during the first $\log{\Delta}$ rounds of phase $i$,
at least $\Omega\left(\frac{m}{\log{n}\log{\Delta}}\right)$ neighbors of nodes in $L$ in $G'$
participate in a productive connection.
\label{lem:match} 
\end{lemma}
 \begin{proof}[Proof Notes]
The original version of this theorem from~\cite{ghaffari:2016} 
requires that $G'$ is a bipartite graph. 
This follows in our case because it is a subset of a productive subgraph.
All subsets of productive subgraphs are bipartite as you can put the nodes
with sender status in one bipartition and nodes with receiver status in the other
(by definition the only edges in a productive subgraph are between sender and receiver nodes).

Another difference is that our theorem studies our gossip
algorithm, while the theorem from~\cite{ghaffari:2016} studies the PPUSH rumor spreading process.
The PPUSH process assumes  a single rumor spreading in the system.
Some nodes know the rumor (and are called {\em informed}) and some nodes do not (and are called {\em uninformed}).
In each round, each node declares whether or not they are uninformed.
Each informed node randomly chooses an uninformed neighbor (if any such neighbors exist)
and tries to form a connection, changing the receiver's status to informed.

The original version of the theorem states that if you execute PPUSH for $\log{\Delta}$
rounds, at least $\Omega(\frac{m}{\log{n}\log{\Delta}})$ nodes that neighbor $L$ are informed.
If we consider senders to be informed and receivers to be uninformed, 
our gossip algorithm behaves the same as PPUSH in $\log{\Delta}$ rounds under consideration.
That is, the senders in $L$ will randomly select a receiver neighbor to attempt a connection.

Once a receiver in $G'$ participates in a connection in our algorithm,
it sets its $done$ flag to $1$ for the remainder of the phase,
preventing future attempts to connect to it during the phase.
This matches the behavior in PPUSH where once a node becomes informed,
informed neighbors stop trying to connect to it.
This congruence allows us to derive the same $\Omega(\frac{m}{\log{n}\log{\Delta}})$ bound
derived for PPUSH in~\cite{ghaffari:2016}.
 \end{proof}
 
 We now combine Lemmas~\ref{lem:prod} and~\ref{lem:match}
 to derive our main result for this part of the analysis.
 
 
\begin{lemma}
Fix some phase $i$.
Let $t= t^*(r_i)$.
With constant probability,
the number of productive connections in this phase is in
$\Omega\left(\frac{\alpha n^*_t(r_i)}{\log{n}\log{\Delta}}\right)$.
\label{lem:progress}
\end{lemma}
 \begin{proof}
 Fix some phase $i$.
 By Lemma~\ref{lem:prod},
 with some constant probability $p_1$,
 the productive subgraph $G_{r_i}$ has a matching
 $M_i$ of size $m_i \geq (\alpha/16)n^*_t(r_i)$
 once nodes randomly set their $status$ flags.
 
 Now consider the subgraph graph $G'$ that consists of every sender
 endpoint in $M_i$,
 and for each such sender $u$,
 every receiver $v$ that neighbors $u$,
 as well as the edge $\{u,v\}$.
 This subgraph satisfies the conditions of Lemma~\ref{lem:match} for $m=m_i$.
 Applying this lemma, it follows that with some constant probability $p_2$,
 during this phase, the random neighbor selections by senders
 will generate at least $\Omega(m_i/(\log{n}\log{\Delta}))$
 productive connections.
 
 Combining these two results,
 we see that with constant probability $p=p_1p_2$,
 we have at least $\Omega(\frac{\alpha n^*_t(r_i)}{\log{n}\log{\Delta}})$ productive connections, 
 as claimed by the lemma statement.
 \end{proof}

\paragraph{The Size Band Table}
In the previous part of this analysis, we
proved that with constant probability the number of productive connections in phase
$i$ is bounded with respect to the number of nodes that know $t^*(r_i)$.
In the worst case, however, $t^*(r_i)$ might be quite small (e.g., at the beginning
of an execution where each token is known by only a constant number of nodes,
this value is constant). We must, therefore, move beyond a worst-case application
of Lemma~\ref{lem:progress}, and amortize the progress over time to something more
substantial.







To accomplish this goal, we introduce a data structure---a tool used only in the context of our analysis---that we
call a {\em size band table}, which we denote as ${\cal S}$.
This table has one column for each token $t\in T$,
and $2\log{(n/2)}+1$ rows which we number $1,2,...,2\log{n/2}+1$.

As we will elaborate below, each row is associated with a range of values that
we call a {\em band}.
We call rows $1$ through $\log{(n/2)}$  {\em growth bands},
and rows $\log{(n/2)} + 1$ through $2\log{(n/2)}+1$ {\em shrink bands}.
Each cell in ${\cal S}$  contains a single bit.
We update these bit values after every round of our gossip algorithm
to reflect the extent to which each token has spread in the system.

In more detail, for each round $r \geq 1$,
we use ${\cal S}_r$ to describe the size band table at the beginning of round $r$.
For each token $t\in T$ and row $i, 1 \leq 1 \leq 2\log{(n/2)}+1$,
we use ${\cal S}_r[t,i]$ to refer to the bit value in row $i$
of the column dedicated to token $t$ in the table for round $r$.

Finally, we define each of these bit values as follows.
For each round $r \geq 1$,
token $t\in T$, and
growth band $i$ (i.e., for each $i, 1 \leq i \leq \log{(n/2)}$),
we define:

\[
{\cal S}_r[t,i] = \begin{cases}
			%1 & \text{if at least $2^i$ nodes know token $t$ at the beginning of round $r$} \\
			1 & \text{if at least $2^i$ nodes know}\\ 
			    & \text{token $t$ at the beginning of round $r$,} \\
			0 & \text{else.}
			\end{cases}
\]

Symmetrically,
for each round  $r \geq 1$,
token $t\in T$, and
shrink band $i$ (i.e., for each $i, \log{(n/2)} + 1 \leq i \leq 2\log{(n/2)} + 1$),
we define:

\[
{\cal S}_r[t,i] = \begin{cases}
			1 & \text{if less than $\frac{n}{2^{i-\log{(n/2)}}}$ nodes do {\em not}}\\
			    & \text{know token $t$ at the beginning of round $r$,} \\
			0 & \text{else.}
			\end{cases}
\]





A key property of the side band table is that as a given token $t$ spreads,
the cells in its column with $1$ bits grow from the smaller rows toward the larger rows. 
That is, if row $i$ is $1$ at the beginning of a given round,
all smaller rows for that token are also $1$ at the beginning of that round.
Furthermore, because nodes never lose knowledge of a token, once a cell is set
to $1$, it remains $1$.

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.45\textwidth]{sizebandtable.pdf}}
\caption{An example size band table for token set $T=\{t_1,t_2,t_3,t_4,t_5\}$ and network size $n=32$.
There is one column for each token. The largest row containing a $1$ for a given token
bounds the token spread.
Token $t_1$, for example, has spread to at least $4$ out of the $32$ nodes,
while token $t_5$ is known to all but $1$ node (indicating that it has spread to at least $31$).
In this example table, token $t_3$, which is spread to somewhere between $16$ to $24$ nodes,
 has the biggest potential to spread in the current round}
\label{fig}
\end{figure}

When all rows for a given token $t$ are set to $1$, it follows that
all nodes know $t$.
This follows because the definition of shrink band $i=2\log{(n/2)}+1$ being set to $1$ 
is that the number of nodes that do {\em not} know $t$ is strictly {\em less}
than:

\begin{eqnarray*}
\frac{n}{2^{i-\log{(n/2)}}} & = & \frac{n}{2^{2\log{(n/2)} + 1 -\log{(n/2)}}}  \\
 &=&  
\frac{n}{2^{\log{(n/2)} + 1}} \\
&=& \frac{n}{2^{\log{(n/2)}} \cdot 2^1} \\
&=& 1.
\end{eqnarray*}


\paragraph{Amortized Analysis of Size Band Table Progress}
As the size band table increases the number of $1$ bits,
we say it {\em progresses} toward a final state of all $1$ bits.
Here we perform an amortized analysis of size band table progress.


To do so, we introduce some notation.
For each phase $i$,
and token $t\in T$,
let $b_t(i)$ be the largest row number that contains a $1$ in $t$'s column in ${\cal S}_{r_i}$.
We call this the {\em current band} for token $t$ in phase $i$.

Let $a(i) = |b_{t^*(r_i)}(i) - \log{(n/2)}|$ define the distance from 
the current band of token $t^*(r_i)$ to the center row number $\log{(n/2)}$.
By the definition of $t^*(r_i)$,
no token has a current band closer to $\log{(n/2)}$ than $t^*(r_i)$ at the start of phase $i$.
We say that phase $i$ is {\em associated} with the current band for $t^*(r_i)$.

Finally, for a given phase $i$, with $t=t^*(r_i)$,
we say this phase is {\em successful} if the number of productive connections
during the phase is at least as large as the lower bound specified by Lemma~\ref{lem:progress};
i.e., there are at least $\frac{\gamma \alpha n^*_{t}(r_i)}{\log{n}\log{\Delta}}$ productive connections.
where $\gamma>0$ is the constant hidden in the asymptotic bound in the lemma statement.

%
%It is important to notice the relationship between $n^*_{t}(r_i)$ and the current band for $t$.
%By definition, $n^*_{t}(r_i) = \Theta(2^{\log{(n/2)} - a(i)})$.
% \note{Do a really good diagram in power point of size band table progressing so that this can be more intuitive for the reader.}

Our first goal in this part of the analysis,
 is to bound the number of successful phases that can be associated with each band.
To do so, we differentiate between two different types of successful phases,
and then bound each separately.

\begin{definition}
Fix some phase $i$ that is associated with some band $j$ at distance $a(i)$ from the center of the size band table.
We say phase $i$ is an {\em upgrade} phase if there exists a subset of the productive connections during phase $i$
that push some token $t$'s current band to a position $j'$ with $|\log{(n/2)} - j'| < a(i)$.
If a phase is not an upgrade phase,
and at least one node is missing at least one token, we call it a {\em fill} phase.
\end{definition}

Stated less formally, we call a phase an upgrade phase if it pushes some token's count closer to the center of the size band
table---row $\log{(n/2)}$---than the band associated with the phase. Our definition is somewhat subtle in that it must handle the case where during a phase a token count
does grow to be closer to the center of the size band table, but then its count continues to grow until it pushes {\em more than} distance $a(i)$ above
the center. We still want to count this as an upgrade phase (hence the terminology about there existing some {\em subset} of the connections
that push the count closer).

Our goal is to bound the number of successful phases possible before all tokens are spread.
We begin with bound on upgrade phases (which hold whether or not
the phase is successful). Our subsequent bound on fill phases, however, considers only successful phases.

\begin{lemma}
There can be at most $k(2\log{(n/2)} + 1)$ upgrade phases.
\label{lem:phase1}
\end{lemma}
\begin{proof}
Fix some band $j$.
Consider an upgrade phase $i$ that is associated with $j$.
By the definition of an upgrade phase, there is some token $t$ with a current band at the start of $i$
that is distance at least $a(i)$ from the center of table, but that has its count grow closer to the center
during the phase. 

We note that it must be the case that $t$'s current band at the start of phase $i$ is a growth band.
This holds because if $t$'s current band is a shrink band then additional spreading of token $t$ can
only {\em increase} its distance from the center of the size band table.

If $j$ is a growth band, then it follows that $t$'s current band starts phase $i$ no larger than $j$ and
ends phase $i$ larger, because current bands for a token never decrease.
Moving forward, therefore, token $t$ can never again be the cause of a phase associated with band $j$ to be categorized as an upgrade phase.

On the other hand, if $j$ is a shrink band,
we know that after phase $i$, 
token $t$'s distance will remain closer to the center of the table than $j$ until $t$'s current band becomes a shrink band.
Once again, therefore, moving forward token $t$ can never again cause a phase associated with band $j$ to be categorized as an upgrade.

The lemma statement follows as
there are  $2\log{(n/2)} + 1$ bands,
and for each band, each of the $k$ tokens can transform that band into an upgrade phase at most once.
\end{proof}

We now bound the number of successful fill phases.
%This argument captures one of the main uses of the size band table as an analytical tool.
To do so, we note that the number of fill phases associated with a given band is bounded by the
worst case number of connections needed before some token's count must advance past that band.
For bands associated with large ranges this worst case number is large.
As shown in the following lemma, however, the number of connections in phases
associated with large bands grows proportionally large as well.
This balancing of growth required and growth obtained is at the core of our amortized analysis.

\begin{lemma}
There can be at most $O((k/\alpha)\log^2{n}\log{\Delta} )$ successful fill phases.
\label{lem:phase2}  
\end{lemma}
\begin{proof}
Consider a group of successful fill phases associated with some band $j$ at distance $a_j$ from the center of the size band table.
Because these are fill phases, the productive connections generated during these phases can never
push some token's count (perhaps temporarily) closer than distance $a_j$ from the center of the table
(any phase in which this occurs becomes, by definition, an upgrade phase).

One way to analyze the distribution of the productive connections during these phases is to consider
a generalization of the size band table in which we record in each cell $[t,i]$ the total number of
productive connections that spread token $t$ while its count falls into the band associated with row $i$.
(Of course, many connections for a given token might occur in a given round, in which we case, we process
them one by one in an arbitrary order while updating the cell counts.) 

If we apply this analysis only for the fill phases fixed above, then we know that the counts in all cells of distance less than
$a_j$ from the center of the table remain at $0$.
By the definition of the size band table, 
for a given token $t$,
the maximum number of connections we can add to cells of distance at least $a_j$ from the center
is loosely upper bounded by $2\cdot 2^{\log{(n/2)} - a_j}$ (the extra factor of two captures
both growth and shrink band cells at least distance $a_j$).
Therefore,
the total number of productive connections we can process into cells at distance at least $a_j$
is at most $2k2^{\log{(n/2)} - a_j}$.

By the definition,
each phase $i$ that is a successful fill phase associated with $j$ generates at least $\frac{\gamma \alpha n^*_{t}(r_i)}{\log{n}\log{\Delta}}$
productive connections, where $t=t^*(r_i)$.
By the definition of $t^*(r_i)$, $t$'s current band is distance $a_j$ from the center.
Therefore, $n^*_{t}(r_i)$ is within a factor of $2$ of $2^{\log{(n/2)} - a_j}$.
By absorbing that constant factor into the constant $\gamma$ (to produce a new constant $\gamma'$),
it follows that this phase generates at least 

\[ z = \frac{\gamma' \alpha 2^{\log{(n/2)} - a_j}}{\log{n}\log{\Delta}}\] 

\noindent new productive connections. Combined with our above upper bound on the total possible productive connections for successful
fill phases associated with $j$, it follows that the total number of successful fill phases associated with $j$ as less than:

\begin{eqnarray*}
z^{-1}2k2^{\log{(n/2)} - a_j} &=&  \left(\frac{\log{n}\log{\Delta}}{\gamma' \alpha 2^{\log{(n/2)} - a_j}}\right) 2k2^{\log{(n/2)} - a_j} \\
 &= & \Theta((k/\alpha)\log{n}\log{\Delta}).
\end{eqnarray*}

We multiply this bound over $2\log{(n/2)} + 1$ possible bands 
to derive $O((k/\alpha)\log^2{n}\log{\Delta})$ total
possible successful fill phases,
providing the bound claimed by the lemma statement.
\end{proof}

\paragraph{Pulling Together the Pieces}
We are now ready to combine the above lemmas to prove our main theorem.

\begin{proof}[Proof (of Theorem~\ref{thm:main})]
Combining Lemmas~\ref{lem:phase1} and~\ref{lem:phase2}, it follows that
there can be at most $\ell = k(2\log{(n/2)} + 1) + O((k/\alpha)\log^2{n}\log{\Delta}) = O((k/\alpha)\log^2{n}\log{\Delta})$ successful
upgrade and fill phases before all $k$ tokens are spread.

By Lemma~\ref{lem:progress},
if the token spreading is not yet complete,
then the probability that the current phase is successful is lower bounded by some constant probability $p>0$.
The actual probability might depend on the execution history up until the current phase,
but the lower bound of $p$ always holds, regardless of this history. 
We can tame these dependencies with a stochastic dominance argument.

In more detail, for each phase $i$ before the tokens are spread, we define a trivial random variable $\hat X_i$ that is $1$ with independent
probability $p$, and otherwise $0$.
Let $X_i$, by contrast, be the random indicator variable that is $1$ if phase $i$ is successful, and otherwise $0$.
For each phase $i$ that occurs after the tokens are spread, $\hat X_i = X_i = 1$ by default.

Note that for each $i$, $X_i$ stochastically dominates $\hat X_i$.
It follows that if $\hat Y_T = \sum_{i=1}^T \hat X_i$ is greater than some $x$ with some probability $\hat p$,
then $Y_T = \sum_{i=1}^T X_i$ is greater than $x$ with probability at least $\hat p$.

With this established, consider the first $T = (c/p)\ell$ phases, for some constant $c\geq 2$.
Note that for this value of $T$, $E[\hat Y_T] = c\ell$.
Because $\hat Y_T$ is the sum of independent random variables,
we concentrate around this expectation. 
In particular, we once again apply the following form of a Chernoff Bound:


\[ \Pr(Y \leq (1-\delta)\mu) \leq e^{- \frac{\delta^2\mu}{2}}, \]

\noindent for $Y=\hat Y_T$, $\delta= 1/2$, and $\mu = c\ell$,
to derive that the probability that $\hat Y_T \leq (c/2)\ell \geq \ell$,
is upper bounded by $e^{-\frac{c\ell}{8}}$.
The same bound therefore holds for the probability that $Y_T \leq (c/2)\ell$.
Notice that this error bound is polynomially small in $n$ with an exponent that grows with constant $c$.
It follows, therefore, that with high probability in $n$,
that token spreading succeeds in the first
$T =  (c/p)\ell = O( (k/\alpha)\log^2{n}\log{\Delta} )$ phases.

To achieve the final {\em round} complexity bound claimed by the theorem statement,
we multiply this upper bound on phases by the length of $\log{N}$ rounds per phase.
\end{proof}

%\newpage

\iffalse
\subsection{Comparison to Existing Solution}


We also achieve $\tilde{O}(k/\alpha)$ for stable graphs in PODC 2017.
But the log factor for that algorithm was $\log^6{n}$ (though we should improve to $\log^5{n}$ since we are now assuming $b=\Omega(\log{n})$.)
It was also a more complicated algorithm in which nodes maintain multiple parallel instances,
each attempting to verify a different guess at the size of $k$ by throwing rumors randomly in bins. 
Only once it converges on the right estimate does it then cycle through parallel instances of rumor
spreading. Lots of overhead. Our algorithm is faster and much more natural and simple and easy to implement.

This algorithm is quite well suited to ongoing communication.
You can introduce a new token anywhere and anytime and it will start spreading.
From an analysis perspective, we no longer have to consider tokens that have spread everywhere.
So in an ongoing scenario the relevant $k$ is just those tokens that are still spreading.

Notice, the PODC 2017 algorithm does not support this. It runs for a given set of $k$ tokens and has no mechanism to tell you
when that collection is done. 
\fi

==> dcoss 2019 -- full version/multipeer.tex <==
\subsection{Peer-to-Peer Networking with the iOS Multipeer Connectivity Framework}
\label{sec:sim:multipeer}
The Multipeer Connectivity (MPC) framework is a library provided by iOS to support  discovery and direct communication with nearby devices. The MPC framework provides a general interface for these peer-to-peer connections, which it implements using lower-level WiFi, peer-to-peer WiFi (WiFi Direct), and/or Bluetooth protocols in a manner that is not exposed to the higher level application.

%In more detail, devices identify themselves with unique identifier objects and form connections through session objects which are identified by a service type (a string with a maximum length of 15 characters). 
%Peers can create or join sessions by creating \emph{browser} and \emph{advertiser} objects, respectively. 

%Once a peer creates a session, it allows interested peers to join and establish a connection. Connections are created over two phases: the discovery phase and session phase, after which connected peers may communicate.

In more detail,
 devices can  create {\em advertiser} objects and use them
 to advertise their interest in forming connections. The advertisements configured through these objects
  include the device's chosen identifier, a service type indicating the sessions it is interested in joining, and a dictionary known as the device's \emph{discovery information} which is bounded to contain no more than 255 bytes when encoded in UTF-8. 
  Simultaneously, devices discover the advertisements from nearby peers by creating
 {\em browser} objects, which can be configured to search for advertisements matching service types of interest.
 
  
%   a session object and a browser object, which represent the type of advertisements the peer is interested in. In addtion to being typed, session objects can be configured to require encryption and to include certificates to allow connecting peers to validate the identity of the peer that created the session.
%    After creating these objects, if the service type of a nearby peer's advertisement matches that of the session, that peer will be discovered. Like communication over connections, discovery of a peer's advertisment is reliable but only after an unspecified amount of time. It is worth noting that peers may also use advertisements even if they have no intention of connecting to other sessions. This behavior is exploited in our implementation so that all devices can constantly broadcast small amounts of status information to their neighbors.

After a device has discovered relevant advertisements from nearby peers through a browser object,
it can then choose to send a {\em connection invitation} to one or more of these advertising peers.
%
% based on the discovery information of these advertisements, the device then may send invitations to these peers. 
 %These invitations contain a reference to a {\em session} object at the originating peer.
These invitations can include some additional data to provide further context. 
Once a peer receives an invitation, it can choose to accept, thereby establishing a shared connection. 
Once connected, a device pair can reliably send and receive data to each other using the connection.
The details of how sent data is partitioned into smaller packets,
and the lower-level protocols used to implement the transmissions, are details that are not exposed to the application.
The MPC framework also provides encryption and certificate options to support secure communication.

Each device maintains a {\em session} object that organizes its connections.
Each session object supports connections with at most $8$ peers.
As mentioned earlier, this restriction on the total number of concurrent connections is a major distinction
between smartphone peer-to-peer networks and those described by many classical peer-to-peer models.


% Each session can support connections to at most 8 peers, 
%  and it provide an interface for sending and receiving data between connected peers. Any of the connected peers may send data at any time to any of the other connected peers, triggering an event on the receiving devices when the data arrives. For large amounts of data, an event is triggered at the receiver to indicate a transmission has begun, allowing the receiver to check in on its progress.
%  The details of how sent data is divided into smaller packets and transmitted is handled by the
%  MPC framework and not exposed to the user.
  
  
 % The data may be sent as a single object or a larger resource partitioned over several Bluetooth data packets, however, the details of the transmission are not exposed to the user. 
  
 Applications interact with the session, advertiser, and browser objects by implementing their respective delegate protocols, which specify the required methods
 and properties that must be implemented by the application to interface properly with the MPC framework. 
 %The implementing delegates are called asynchronously in response to relevant events.
 % which are often the consequence of a call made by the application or a nearby peer to the MPC framework. 
 %This pattern is further explained and leveraged in Section IV-C.

==> dcoss 2019 -- full version/related.tex <==
\section{Related Work}
\label{sec:related}

In recent years, there has been a growing amount of research on smartphone peer-to-peer 
networking~\cite{suzuki2012soscast,aloi2014spontaneous,reina2015survey,lu2016networking,holzer2016padoc,firechat,oghostpot} 
(see~\cite{nishiyama2014relay} for a survey).
%A major factor differentiating this setting from those studied in the voluminous existing literature on ad hoc, mobile ad hoc, and sensor networks,
%is the ubiquity of the platform (there are more than 3.9 billion smartphone subscriptions worldwide~\cite{smartphones}) and the ease of deploying software (through well-established apps stores).
%
There has also been recent work on using device-to-device links to improve cellular network performance, e.g., the inclusion of peer-to-peer connections
in the emerging LTE-advanced standard~\cite{doppler2009device,wang2015energy,liu2015device}, but these efforts differ from the peer-to-peer applications studied here as they typically assume coordination provided by the cellular infrastructure.

%In this paper, we propose rigorously analyzing peer-to-peer algorithms in abstractions such as the mobile telephone model,
%and then using simulation strategies to deploy these algorithms on real smartphones.
In this paper, 
we both study and extend the mobile telephone model  introduced in 2016 by Ghaffari and Newport~\cite{ghaffari:2016}.
This model modifies the classical telephone model of wired peer-to-peer networks (e.g., \cite{frieze1985shortest,telephone1,telephone2,telephone3,giakkoupis2011tight,chierichetti2010rumour,giakkoupis2012rumor,fountoulakis2010rumor,giakkoupis2014tight}) to better match the constraints and capabilities of the smartphone setting.
In particular, the mobile telephone model differs from the classical telephone model in that it allows small advertisements but restricts the number
of concurrent connections at a given node. As agued in~\cite{ghaffari:2016}, these differences (especially the latter) significantly change achievable results,
algorithm strategy, and
analysis techniques. The details of this model are inspired, in particular, but the multipeer connectivity framework offered in iOS.

Our random spread gossip algorithm disseminates $k$ rumors in at most $O((k/\alpha)\log^4{n})$ rounds in the mobile telephone model
in a network with $n$ nodes and vertex expansion $\alpha$ (see Section~\ref{sec:model:vertex}).
The previous best known algorithm for this model is crowded bin gossip~\cite{newport:2017b},
which is significantly more complicated and requires $O((k/\alpha)\log^5{n})$ rounds.\footnote{In~\cite{newport:2017b}, crowded bin
is listed as requiring $O((k/\alpha)\log^6{n})$ rounds, but that result assumes single bit advertisements in each round---requiring devices to spell out
control information over many rounds of advertising. To normalize with this paper,
in which tags can contain $\log{n}$ bits, crowded bin's time complexity improves by a $\log$ factor. We note that~\cite{newport:2017b} also explores slower
gossip solutions for more difficult network settings not considered here; e.g., changing network topologies and the absence of advertisements.}

To put these time bounds into context, 
we note that previous work in the mobile telephone model solved rumor spreading~\cite{ghaffari:2016}
 and leader election~\cite{newport:2017} in $O(\text{polylog}(n)/\alpha)$ rounds.
In the classical telephone model, 
a series of papers~\cite{chierichetti2010rumour,giakkoupis2012rumor,fountoulakis2010rumor,giakkoupis2014tight}  (each optimizing the previous) established that simple random rumor spreading requires $O(\log^2{n}/\alpha)$ rounds~\cite{giakkoupis2014tight},
which is optimal in the sense that for many $\alpha$ values,
there exists networks with a diameter in $\Omega(\log^2{n}/\alpha)$.
%
The fact that our gossip solution increases these bounds by a factor of $k$ (ignoring log factors) is natural
given that we allow only a constant number of tokens to be transferred per round.

As mentioned, random gossip processes more generally have been studied in other network models. These abstractions generally model time as synchronized rounds and by definition require nodes to select a neighbor uniformly at random in each round \cite{boyd2006gossip} \cite{karp2000rumor}. More recent work has demonstrated that these protocols take advantage of key graph properties such as vertex expansion and graph conductance \cite{moskaoyama2006conductance}. Asynchronous variants of these protocols have also been explored, where asynchrony is captured by assigning each node a clock following an unknown but well-defined probability distribution \cite{boyd2006gossip} \cite{giakkoupis2016rumor}.
The asynchronous MTM model introduced in our paper, by contrast, 
deploys a more general and classical approach to asynchrony in which an adversarial scheduler controls the time required for key events in a worst-case fashion.
\iffalse
\note{We need some examples here...look for classical random gossip results...I think they sometimes call the results model the GOSSIP model. Some of the papers cited
above next to ``classical telephone model" might point you in the right direction. Just two or so results might be fine.}
\fi
%Finally, we note that%
%Censor-Hillel et~al.~\cite{censor2012global} provide a more involved algorithm that spreads information
%in $O(D + \text{polylog}(n))$ rounds, regardless of the graph's connectivity.
%This result depends heavily on the assumption of unbounded message size and the ability for a single node
%to service an unbounded number of incoming connections in a single round.
%It is unclear, therefore, whether efficient information dissemination independent of graph connectivity is possible in our model.

%Finally,
%we note that our approach of adapting algorithms from high-level abstractions to real devices through simulation is not the only way to simplify
%smartphone peer-to-peer network design. 
%The Open Garden MeshKit SDK~\cite{meshkit}, for example,
%provides an abstraction layer between the application developer and smartphone peer-to-peer functionality that implements additional useful
%functions, like a global name space and private message routing.
%The Padoc middleware~\cite{holzer2016padoc}, to name another example, 
%extends the Multipeer Connectivity framework to better support background operation,
%among other improvements.

==> dcoss 2019 -- full version/sim.tex <==
\section{Implementing Mobile Telephone Model Algorithms on Real Mobile Phones} \label{sec:sim}

The mobile telephone model abstraction captures the basic discover-and-connect dynamics provided by standard smartphone peer-to-peer libraries.
Algorithms designed for this model, however, cannot be directly deployed on real hardware.
The main issue is synchronization.
Like many abstractions used to study distributed graph algorithms,
the mobile telephone model coordinates network communication in globally synchronized rounds.
Though real smartphones implement the same basic primitives of advertising, discovering, and connecting,
they do not offer synchronous rounds,
and the time required for the basic communication primitives to succeed can vary over an execution and between devices,
complicating simple timeout-based efforts to keep devices coordinated.

To overcome this issue,
we describe and analyze a strategy for simulating the abstract mobile telephone model on real mobile phone hardware.
We focus in particular on implementing this strategy in the Multipeer Connectivity Framework for peer-to-peer networking that has been included
in every iOS release since version 7.
We begin in Section~\ref{sec:sim:multipeer} by summarizing the Multipeer Framework.
Then, in Section~\ref{sec:sim:sim}, we formalize what it means to simulate the mobile telephone model,
and then describe a strategy that does so using this  framework.




\input{multipeer}


\subsection{Simulating the Mobile Telephone Model using the Multipeer Connectivity Framework}
\label{sec:sim:sim}
%We begin with a brief summary of the MTM's behavior (see Section~\ref{sec:mtm} for details).
%The execution then proceeds in synchronous rounds.
%At the beginning of each round $r$, 
%each node $u$  chooses a bounded size advertisement to share with its neighbors,
%and then learns its neighbors' advertisements.
%We can call this the {\em scan} phase of the round.
%After all nodes complete the scan phase,
%they enter the {\em connect} phase of the round.
%During this phase, each node $u$
%can decide whether to send a connection attempt to a neighbor or receive connection attempts.
%If it chooses to receive attempts, it can accept at most one of the incoming attempts, forming a connection.\footnote{Recall
%that the only guarantee provided about incoming connection attempts is that if at least one neighbor of $u$
%sends an attempt then $u$ will receive at least one attempt---it is not guaranteed, for example, that $u$
%gets to receive all connection attempts before making a decision.}
%If $u$ forms a connection with neighbor $v$---either through accepting an attempt or having its attempt connected---nodes
%$u$ and $v$ can perform a bounded amount of reliable communication.
%After all connections are concluded, the connect phase for round $r$ ends and the model moves on to the scan
%phase of round $r+1$.

Here we describe how to simulate the mobile telephone model using the MPC framework.
Our goal is to combine mobile telephone model algorithms with this simulator to enable their execution on real iOS devices,
while maintaining the algorithms' original theoretical guarantees.

We begin by formalizing the problem of simulating the mobile telephone model.
That is, we specify an interface through which the simulation interacts with a mobile telephone model algorithm,
and enumerate the properties these interactions must satisfy to achieve a correct simulation.
We then describe and analyze our strategy for implementing this interface in such a way that it satisfies these properties.


\paragraph{The Mobile Telephone Model Interface}
As detailed in Section~\ref{sec:mtm},
each round in the mobile telephone model can be subdivided into two {\em phases}.
The first is a {\em scan} phase in which nodes choose an advertisement for the round and then scan to discover their neighbors' advertisements.
The second is a {\em connect} phase in which nodes send and receive connection invitations and, if they end up forming a connection, 
participate in a bounded amount of communication.

One way to formalize an algorithm that proceeds through these phases is to specify an interface through which the algorithm coordinates with the underlying 
 model. Here we formalize one such interface
 from the perspective of a node $u$ running mobile telephone model algorithm ${\cal A}$:


\begin{itemize}


	\item {\tt requestAdv}$(r)_u$: This function is implemented by $u$ and called by the model to request
	$u$'s advertisement for the scan phase of round $r$. Node $u$ returns the advertisement as the return value for the function call.
	
	\item {\tt deliverAdv}$(r,A)_u$: This function is implemented by $u$ and called by the model to deliver
	the set $A$ containing all of the round $r$ advertisements of $u$'s neighbors.
	
	\item {\tt endScan}$(r)_u$: This function is implemented by $u$ and called by the model
	to indicate that the scan phase for round $r$ is concluded and $u$ is now free
	to send a connection invitation for this round.
	
	
	\item {\tt endConnect}$(r)_u$: This function is called by $u$ to inform the model that it has completed
	its attempt (if any) to send a connection attempt in round $r$, and if such an attempt was accepted,
	it is also done with the resulting connection. If $u$ decides
	not to send a connection attempt in round $r$, it can immediately call this function after 
	its {\tt endScan} call.
			
\end{itemize}


\paragraph{The Mobile Telephone Model Properties}
We now specify the properties the mobile telephone model must satisfy when interacting with an algorithm through the above interface 
to match the behavior described in Section~\ref{sec:mtm}.

Before defining these properties,
we must first specify what we require from the mobile telephone model algorithm interacting with this interface.
In more detail, we say such an algorithm is {\em well-formed} if it: (a) always responds to {\tt requestAdv} calls with an advertisement;
and (b) only ever attempts connections after the {\tt endScan} call for the round, and correctly calls {\tt endConnect}
after its connection attempt (if any)  for the round completes.

We can now formalize what the model guarantees when interacting with a well-formed algorithm:

\begin{property}
When interacting with a well-formed algorithm ${\cal A}$,
the mobile telephone model satisfies the following guarantees:

\begin{enumerate}
%\item For each node $u$, {\tt deliverNbrs}$(N)_u$ is called at the beginning of the execution where $N$ is the set of $u$'s neighbors.
\item For each round $r\geq 1$ and node $u$,
the model calls {\tt requestAdv}$(r)_u$ and then subsequently calls {\tt deliverAdv}$(r,A)_u$ where $A$ contains,
for each neighbor $v$ of $u$,
the advertisement returned by $v$ for the call {\tt requestAdv}$(r)_v$.
\item For each round $r \geq 1$ and node $u$, the model will call {\tt endScan}$(r)_u$ at some point after it: calls {\tt deliverAdv}$(r,A_u)_u$,
and has called {\tt deliverAdv}$(r,A_v)_v$ for each neighbor $v$ of $u$.
%
%For each neighbor $v$ of $u$, however,
%the model will not call {\tt endScan}$(r)_v$ until {\em after} it calls {\tt deliverAdv}$(r,A)_u$.

\item For each round $r > 1$ and node $u$,
the model will {\em not} call {\tt requestAdv}$(r)_u$ until after every node $v$ in the set containing $u$, and all of $u$'s neighbors,
has already called {\tt endConnect}$(r-1)_v$.

\end{enumerate}
%
\label{prop:mtm}
\end{property}

It is straightforward to establish that a model that interacts with a well-formed algorithm through
the mobile telephone interface, and satisfies the guarantees of Property~\ref{prop:mtm}, implements the same model
behavior described in Section~\ref{sec:mtm}.

The first property requires the model to correctly collect and deliver advertisements for each round.

The second property requires the model to eventually shift each node $u$ from the scan to connect phase in each round,
but to wait before doing so until all of $u$'s neighbors have also already received their advertisements for the round.
This latter property is necessary because it guarantees that if a node $u$ sends a connection invitation to neighbor $v$,
this neighbor has already received its advertisements for the round.

The third property requires for each node $u$ and round $r$,
that all connection behavior involving $u$ for round $r$ is complete before $u$ moves on to 
decide an advertisement for round $r+1$.
That is, not only has $u$ completed any attempted connections,
but all of $u$'s neighbors have also completed any attempted connections (including, importantly, connection invitations sent to $u$).

\paragraph{The MTM Sim Algorithm}
Our final step is to describe and analyze a strategy that implements the model interface and properties
described above using the MPC framework.
We call this strategy MTM sim (short for: mobile telephone model simulation).
We describe it below from
the perspective of a node $u$ that is using MTM sim to simulate some well-formed
mobile telephone model algorithm ${\cal A}$.



\begin{itemize}


%\begin{quote}{\bf simMTM Algorithm (simulating MTM for algorithm ${\cal A}$ on node $u$).}
\item At the beginning of each simulated round $r$,
the MTM sim algorithm calls the {\tt requestAdv}$(r)_u$ function implemented by ${\cal A}$ to learn $a_u(r)$: the advertisement generated by ${\cal A}$ for $u$ in simulated round $r$.
The algorithm updates $u$'s MPC framework advertisement to $\langle r, a_u(r), 0,0\rangle$.\footnote{We omit the requirement here for a node to include its
id in its advertisement. With the MPC framework you always learn the identify of the node that generated a discovered advertisement, so including it
in the advertisement payload is redundant.}

%The algorithm sets $u$'s advertisement to $\langle r, a_u(r), 0,0\rangle$.
%The first $0$ bit indicates (roughly speaking) that $u$ is not yet ready to end the scan phase of this round.
%The second $0$ bit indicates (roughly speaking) that $u$ is not yet ready to end the connect phase.

\item The MTM sim algorithm then blocks until it has learned the simulated round $r$ advertisement (i.e., as delivered in an MPC advertisement
 of  the form  $\langle r, *, *,*\rangle$) from each of $u$'s neighbors in the network.
At this point, the  algorithm does two things:  (1) it calls {\tt deliverAdv}$(r,A)_u$, where $A$ is the set of its neighbors'  advertisements for simulated $r$; and
  (2) it changes $u$'s MPC advertisement to $\langle r, a_u(r), 1,0\rangle$.

\item The MTM sim algorithm then blocks 
 until all of $u$'s neighbors have a $1$ in the third field of their MPC advertisement.
 At this point, it calls {\tt endScan}$(r)_u$.
 
 \item The MTM sim algorithm blocks until algorithm ${\cal A}$ running on $u$ calls {\tt endConnect}$(r)_u$. At this point,
MTM sim updates $u$'s MPC advertisement to $\langle r, a_u(r), 1,1\rangle$.
 
 \item The MTM sim algorithm blocks until all neighbors of $u$ include a $1$ in the fourth field of their MPC advertisement.
 At this point, it advances to simulated round $r+1$.
  
\end{itemize} 

Notice, it is possible that a node might miss an advertisement that it is waiting to receive during one of the blocking steps.
This can occur if a neighbor of some node $u$ changes its advertisement too quickly for $u$ to discover it.

To compensate for this possibility,
we assume our above algorithm {\em reconstructs} missed advertisements.
That is, if $u$ notices that it missed an advertisement from its neighbor $v$,
it reconstructs the missing advertisement based on the current advertisement it sees from $v$.
It then simulates first receiving the reconstructed advertisement before the current advertisement.
The core of the below correctness proof
is an argument that each node $u$ can fall behind at most one advertisement for a given neighbor.
A case analysis on the advertisement type then establishes that
 it is always possible to reconstruct the missed advertisement in this case.

\begin{theorem}
When executed with a well-formed  algorithm,
the MTM sim algorithm satisfies the mobile telephone model guarantees defined by Property~\ref{prop:mtm}.
%Furthermore, 
%for every round $r\geq 1$,
%node $u$,
%the MTM sim algorithm requires at most $O(r\cdot \hat t)$ time to simulate the first $r$ rounds for $u$,
%where $\hat t$ is the worst case time for a node to 
%
% = \delta_a + 2\delta_i + \delta_m$ is the round length.
\label{thm:mtm}
\end{theorem}
% [space cut]
\iffalse
\begin{proof}
We begin by studying MTM sim under the simplifying assumption
that no advertisements are missed.
That is,
if a node $u$ updates its advertisement to $a$, then all neighbors of $u$ learn of this update,
even if the interval between this update and $u$'s subsequent update is small.
Under this assumption,
the correctness of MTM sim is easy to establish as its operations directly implement the guarantees of Property~\ref{prop:mtm}.

As noted in the algorithm description, however,
it is possible that some advertisements are missed; e.g., $u$ updates to $a$, and then to $a'$ so fast
that some neighbor $v$ does not have enough time to discover $a$.
In this case, as described, the MTM sim algorithm attempts to reconstruct the missed advertisement.
To conclude this proof, we must show that this reconstruction is always possible,
which implies the nodes running MTM sim are simulating the above assumption of no missed advertisements.

To make this argument, we note that the we can place the MPC advertisement types used by MTM sim into a total order; i.e.,

\[ \langle 1, *, 0,0\rangle,  \langle 1, *, 1,0\rangle,  \langle 1, *, 1,1\rangle,\]  
\[\langle 2, *, 0,0\rangle,  \langle 2, *, 1,0\rangle, 
 \langle 2, *, 1,1\rangle, \langle 3, *, 0,0\rangle...\]

A useful property of the MTM sim algorithm is that if at a given point in an execution
a node $u$ is currently advertising the type in some position $i>1$ in the above total order,
then it must be the case that prior to this point all of $u$'s neighbors advertised the type in position $i-1$,
as this is required by the algorithm for $u$ to advance to the next advertisement type.

To apply this property, consider some node $v$ and some point in the execution
at which $v$ is advertising the type in some position $i \geq 1$.
For each neighbor $u$ of $v$,
$u$ can only be at most one advertisement type ahead of $v$. That is, it is possible that $u$
is advertising the type in position $i+1$ at this point, but it cannot be advertising
a type in a position strictly greater than $i+1$, as this would require a later advertisement type from $v$.
Furthermore, because $v$ is at position $i$, it must already know $u$'s type $i-1$ advertisement,
as this was required for $v$ to advance to position $i$.

In this case, it is possible that $v$ missed one advertisement from $u$.
That is, that $v$ missed $u$'s position $i$ advertisement as $u$ moved
from $i$ to $i+1$.
If this occurs $v$ will remain in $i$, and therefore $u$ will remain at type $i+1$,
until after $v$ is able to reconstruct $u$'s position $i$ advertisement.
It follows that $v$ will eventually hear $u$'s type $i+1$ advertisement and can use this to aid its reconstruction.

A simple case analysis on the advertisement types establishes that if $v$ knows $u$'s type $i-1$ advertisement
{\em and} its type $i+1$ advertisement, then $v$ has all of the information it needs
to reconstruct $u$'s type $i$ advertisement.
\end{proof}
\fi

We are left to bound the time complexity overhead generated by the MTM sim algorithm.
To do so, let the {\em round length} $\hat t$ be the worst case time required by the MPC framework
for any node to implement all three of the following steps: (1) update its advertisement and have all neighbors discover the update; (2) send a connection invitation
and have it accepted; and (3) send over the connection the bounded amount of information allowed in a single round of the mobile telephone model.
Clearly, $r\cdot \hat t$ is a worst-case lower bound on the time required to simulate $r$ mobile telephone model rounds,
as each such simulated round requires advertising, discovery, invitations, and (potentially) a connection.




\iffalse
%That is, we bound the worst case time required for a given node to complete the simulation of a given MTM round (i.e., the
%time between two consecutive {\tt requestAdv} calls). 

To do so, let $\delta_{m}$ be the maximum amount of time required to complete the bounded amount of communication
allowed during a connection in the MTM (this is a function of the bound on allowed communication and the slowest possible
bit rate $r_{max}$ at which this communication might occur). We define the {\em round length} $\hat t = \delta_a + 2\delta_i + \delta_m$.
(Recall from Section~\ref{sec:pmtm} that $\delta_a$ and $\delta_b$ are the maximum times to 
spread a new advertisement to all your neighbors and send/reply to a connection attempt, respectively.)

The round length $\hat t$ is therefore the worst case time required for a pair of nodes to hear each others' advertisements and then
form a connection. 
It follows that $\hat t$ provides an obvious lower bound for the worst case time required to simulate a given round of the MTM model.
Here we prove that in the worst case, simMTM requires $O(r\cdot \hat t)$ time to simulate $r$ rounds; i.e., 
the average time per round is within a constant factor of the obvious lower bound.\footnote{We emphasize that this result 
is not necessarily expected. The simMTM algorithm requires nodes to collect advertisements of a certain type from
all of their neighbors before moving on to the next type. It is plausible, therefore, the network might generate over time a chain
of dependencies. For example, imagine a line network in which we label the nodes $1,2,3...,n$. Imagine each node $i >1$
is waiting on an advertisement from its neighbor $i-1$ of the type in position $i-1$ of the total ordering used
in the proof of Theorem~\ref{thm:mtm}. This creates a chain of dependencies until we have to wait for
$i$ to update its type before $i+1$. The total time until node $n$ makes progress, therefore, is now a function
of the network size. We leverage a classical result from the study of synchronizers to show such chains
take a long time to establish and the average time per round therefore remains efficient.}
\fi

Our goal is to prove that the MTM sim strategy matches this lower bound within constant factors.
Fortunately, this property follows by noting that the advertisement blocking implemented by MTM sim is a standard
local synchronization strategy, and then applying the
 classical results on local synchronization first implied by Gallager~\cite{gallager:1982} and Awerbuch~\cite{awerbuch:1985},
 and later formalized by Lynch~\cite{nancytextbook} in  Section 16.2). Formally:



%a simple synchronizer strategy in which nodes in an asynchronous message passing model must send and collect
%round $i$ messages from each neighbor before sending a round $i+1$ message, requires, for each count $r\geq 1$,
%$O(r(d+\ell))$ time to get all nodes up to round $r$,
%where $d$ is an upper bound on message delay and $\ell$ is an upper bound on the 
%ocal steps at a given node required for each round.

%By equating each advertisement type as a round in the classical synchronizer
%result, and noting in this context the delay between subsequent advertisement types is bounded by $O(\hat t)$, implying $d+\ell = O(\hat t)$, 
%the following holds:

\begin{theorem}
For any $r\geq 1$,
node $u$, and MPC round length $\hat t$,
the MTM sim algorithm requires $O(r\cdot \hat t)$ time to simulate the first $r$ rounds for $u$.
\label{thm:time}
\end{theorem}


\paragraph{Tolerating Network Changes}
We conclude by noting that the MTM sim algorithm as described is not particularly fault-tolerant.
If a neighbor of $u$ crashes or leaves the area, for example, 
$u$ will block indefinitely waiting for $u$'s next anticipated advertisement type.
A straightforward heuristic to accommodate this possibility is to implement a simple time out mechanism: if $u$ fails
to hear from neighbor $v$ for sufficiently long, $u$ removes $v$ from its list of neighbors.


Similarly, if node $u$ hears an advertisement of a {\em new} neighbor $v$,
it can add $v$ to its neighbor list starting with an upcoming round.
If node $v$ was a neighbor that $u$ recently removed due to a time out, it might conclude that
its time out value is too small and increase it---allowing it to adapt to the current network conditions.
%
More generally, we note that identifying optimal heuristics for tolerating network changes is important
future work to help advance this research direction.

\iffalse

Finally, we note that when a node $u$ joins a network for the first time,
or migrates from one network partition to another,
it might discover that its new neighbors are far ahead or behind in their rounds. 
In this case, $u$ can make a discontinuous jump to the local round to allow it to proceed with it neighbors going forward.
It might therefore make sense in this case to add a {\tt roundAdjust}$(r,r')$ function to the mobile telephone model interface
to provide algorithms a way to be notified that a round jump occurred.
Such jumps have little effect on our random spread gossip algorithm,
but other algorithms might require specific action to recover from such changes.

We leave the details of identifying the best possible modifications to MTM sim to tolerate changing networks
as interesting future work. 

\fi








==> gossipProblem.tex <==
\subsection{The Gossip Problem}

% Motivate our study of the gossip problem in p2p networks
% Describe the gossip problem
% Give trivial algorithms that take O(kn) rounds and mention 2017 PODC results

==> multipeer.tex <==
\subsection{Peer-to-Peer Networking with the iOS Multipeer Connectivity Framework}
\label{sec:sim:multipeer}
The Multipeer Connectivity (MPC) framework is a library provided by iOS to support  discovery and direct communication with nearby devices. The MPC framework provides a general interface for these peer-to-peer connections, which it implements using lower-level WiFi, peer-to-peer WiFi (WiFi Direct), and/or Bluetooth protocols in a manner that is not exposed to the higher level application.

%In more detail, devices identify themselves with unique identifier objects and form connections through session objects which are identified by a service type (a string with a maximum length of 15 characters). 
%Peers can create or join sessions by creating \emph{browser} and \emph{advertiser} objects, respectively. 

%Once a peer creates a session, it allows interested peers to join and establish a connection. Connections are created over two phases: the discovery phase and session phase, after which connected peers may communicate.

In more detail,
 devices can  create {\em advertiser} objects and use them
 to advertise their interest in forming connections. The advertisements configured through these objects
  include the device's chosen identifier, a service type indicating the sessions it is interested in joining, and a dictionary known as the device's \emph{discovery information} which is bounded to contain no more than 255 bytes when encoded in UTF-8. 
  Simultaneously, devices discover the advertisements from nearby peers by creating
 {\em browser} objects, which can be configured to search for advertisements matching service types of interest.
 
  
%   a session object and a browser object, which represent the type of advertisements the peer is interested in. In addtion to being typed, session objects can be configured to require encryption and to include certificates to allow connecting peers to validate the identity of the peer that created the session.
%    After creating these objects, if the service type of a nearby peer's advertisement matches that of the session, that peer will be discovered. Like communication over connections, discovery of a peer's advertisment is reliable but only after an unspecified amount of time. It is worth noting that peers may also use advertisements even if they have no intention of connecting to other sessions. This behavior is exploited in our implementation so that all devices can constantly broadcast small amounts of status information to their neighbors.

After a device has discovered relevant advertisements from nearby peers through a browser object,
it can then choose to send a {\em connection invitation} to one or more of these advertising peers.
%
% based on the discovery information of these advertisements, the device then may send invitations to these peers. 
 %These invitations contain a reference to a {\em session} object at the originating peer.
These invitations can include some additional data to provide further context. 
Once a peer receives an invitation, it can choose to accept, thereby establishing a shared connection. 
Once connected, a device pair can reliably send and receive data to each other using the connection.
The details of how sent data is partitioned into smaller packets,
and the lower-level protocols used to implement the transmissions, are details that are not exposed to the application.
The MPC framework also provides encryption and certificate options to support secure communication.

Each device maintains a {\em session} object that organizes its connections.
Each session object supports connections with at most $8$ peers.
As mentioned earlier, this restriction on the total number of concurrent connections is a major distinction
between smartphone peer-to-peer networks and those described by many classical peer-to-peer models.


% Each session can support connections to at most 8 peers, 
%  and it provide an interface for sending and receiving data between connected peers. Any of the connected peers may send data at any time to any of the other connected peers, triggering an event on the receiving devices when the data arrives. For large amounts of data, an event is triggered at the receiver to indicate a transmission has begun, allowing the receiver to check in on its progress.
%  The details of how sent data is divided into smaller packets and transmitted is handled by the
%  MPC framework and not exposed to the user.
  
  
 % The data may be sent as a single object or a larger resource partitioned over several Bluetooth data packets, however, the details of the transmission are not exposed to the user. 
  
 Applications interact with the session, advertiser, and browser objects by implementing their respective delegate protocols, which specify the required methods
 and properties that must be implemented by the application to interface properly with the MPC framework. 
 %The implementing delegates are called asynchronously in response to relevant events.
 % which are often the consequence of a call made by the application or a nearby peer to the MPC framework. 
 %This pattern is further explained and leveraged in Section IV-C.

==> sim.tex <==
\section{Implementing Mobile Telephone Model Algorithms on Real Mobile Phones} \label{sec:sim}

The mobile telephone model abstraction captures the basic discover-and-connect dynamics provided by standard smartphone peer-to-peer libraries.
Algorithms designed for this model, however, cannot be directly deployed on real hardware.
The main issue is synchronization.
Like many abstractions used to study distributed graph algorithms,
the mobile telephone model coordinates network communication in globally synchronized rounds.
Though real smartphones implement the same basic primitives of advertising, discovering, and connecting,
they do not offer synchronous rounds,
and the time required for the basic communication primitives to succeed can vary over an execution and between devices,
complicating simple timeout-based efforts to keep devices coordinated.

To overcome this issue,
we describe and analyze a strategy for simulating the abstract mobile telephone model on real mobile phone hardware.
We focus in particular on implementing this strategy in the Multipeer Connectivity Framework for peer-to-peer networking that has been included
in every iOS release since version 7.
We begin in Section~\ref{sec:sim:multipeer} by summarizing the Multipeer Framework.
Then, in Section~\ref{sec:sim:sim}, we formalize what it means to simulate the mobile telephone model,
and then describe a strategy that does so using this  framework.




\input{multipeer}


\subsection{Simulating the Mobile Telephone Model using the Multipeer Connectivity Framework}
\label{sec:sim:sim}
%We begin with a brief summary of the MTM's behavior (see Section~\ref{sec:mtm} for details).
%The execution then proceeds in synchronous rounds.
%At the beginning of each round $r$, 
%each node $u$  chooses a bounded size advertisement to share with its neighbors,
%and then learns its neighbors' advertisements.
%We can call this the {\em scan} phase of the round.
%After all nodes complete the scan phase,
%they enter the {\em connect} phase of the round.
%During this phase, each node $u$
%can decide whether to send a connection attempt to a neighbor or receive connection attempts.
%If it chooses to receive attempts, it can accept at most one of the incoming attempts, forming a connection.\footnote{Recall
%that the only guarantee provided about incoming connection attempts is that if at least one neighbor of $u$
%sends an attempt then $u$ will receive at least one attempt---it is not guaranteed, for example, that $u$
%gets to receive all connection attempts before making a decision.}
%If $u$ forms a connection with neighbor $v$---either through accepting an attempt or having its attempt connected---nodes
%$u$ and $v$ can perform a bounded amount of reliable communication.
%After all connections are concluded, the connect phase for round $r$ ends and the model moves on to the scan
%phase of round $r+1$.

Here we describe how to simulate the mobile telephone model using the MPC framework.
Our goal is to combine mobile telephone model algorithms with this simulator to enable their execution on real iOS devices,
while maintaining the algorithms' original theoretical guarantees.

We begin by formalizing the problem of simulating the mobile telephone model.
That is, we specify an interface through which the simulation interacts with a mobile telephone model algorithm,
and enumerate the properties these interactions must satisfy to achieve a correct simulation.
We then describe and analyze our strategy for implementing this interface in such a way that it satisfies these properties.


\paragraph{The Mobile Telephone Model Interface}
As detailed in Section~\ref{sec:mtm},
each round in the mobile telephone model can be subdivided into two {\em phases}.
The first is a {\em scan} phase in which nodes choose an advertisement for the round and then scan to discover their neighbors' advertisements.
The second is a {\em connect} phase in which nodes send and receive connection invitations and, if they end up forming a connection, 
participate in a bounded amount of communication.

One way to formalize an algorithm that proceeds through these phases is to specify an interface through which the algorithm coordinates with the underlying 
 model. Here we formalize one such interface
 from the perspective of a node $u$ running mobile telephone model algorithm ${\cal A}$:


\begin{itemize}


	\item {\tt requestAdv}$(r)_u$: This function is implemented by $u$ and called by the model to request
	$u$'s advertisement for the scan phase of round $r$. Node $u$ returns the advertisement as the return value for the function call.
	
	\item {\tt deliverAdv}$(r,A)_u$: This function is implemented by $u$ and called by the model to deliver
	the set $A$ containing all of the round $r$ advertisements of $u$'s neighbors.
	
	\item {\tt endScan}$(r)_u$: This function is implemented by $u$ and called by the model
	to indicate that the scan phase for round $r$ is concluded and $u$ is now free
	to send a connection invitation for this round.
	
	
	\item {\tt endConnect}$(r)_u$: This function is called by $u$ to inform the model that it has completed
	its attempt (if any) to send a connection attempt in round $r$, and if such an attempt was accepted,
	it is also done with the resulting connection. If $u$ decides
	not to send a connection attempt in round $r$, it can immediately call this function after 
	its {\tt endScan} call.
			
\end{itemize}


\paragraph{The Mobile Telephone Model Properties}
We now specify the properties the mobile telephone model must satisfy when interacting with an algorithm through the above interface 
to match the behavior described in Section~\ref{sec:mtm}.

Before defining these properties,
we must first specify what we require from the mobile telephone model algorithm interacting with this interface.
In more detail, we say such an algorithm is {\em well-formed} if it: (a) always responds to {\tt requestAdv} calls with an advertisement;
and (b) only ever attempts connections after the {\tt endScan} call for the round, and correctly calls {\tt endConnect}
after its connection attempt (if any)  for the round completes.

We can now formalize what the model guarantees when interacting with a well-formed algorithm:

\begin{property}
When interacting with a well-formed algorithm ${\cal A}$,
the mobile telephone model satisfies the following guarantees:

\begin{enumerate}
%\item For each node $u$, {\tt deliverNbrs}$(N)_u$ is called at the beginning of the execution where $N$ is the set of $u$'s neighbors.
\item For each round $r\geq 1$ and node $u$,
the model calls {\tt requestAdv}$(r)_u$ and then subsequently calls {\tt deliverAdv}$(r,A)_u$ where $A$ contains,
for each neighbor $v$ of $u$,
the advertisement returned by $v$ for the call {\tt requestAdv}$(r)_v$.
\item For each round $r \geq 1$ and node $u$, the model will call {\tt endScan}$(r)_u$ at some point after it: calls {\tt deliverAdv}$(r,A_u)_u$,
and has called {\tt deliverAdv}$(r,A_v)_v$ for each neighbor $v$ of $u$.
%
%For each neighbor $v$ of $u$, however,
%the model will not call {\tt endScan}$(r)_v$ until {\em after} it calls {\tt deliverAdv}$(r,A)_u$.

\item For each round $r > 1$ and node $u$,
the model will {\em not} call {\tt requestAdv}$(r)_u$ until after every node $v$ in the set containing $u$, and all of $u$'s neighbors,
has already called {\tt endConnect}$(r-1)_v$.

\end{enumerate}
%
\label{prop:mtm}
\end{property}

It is straightforward to establish that a model that interacts with a well-formed algorithm through
the mobile telephone interface, and satisfies the guarantees of Property~\ref{prop:mtm}, implements the same model
behavior described in Section~\ref{sec:mtm}.

The first property requires the model to correctly collect and deliver advertisements for each round.

The second property requires the model to eventually shift each node $u$ from the scan to connect phase in each round,
but to wait before doing so until all of $u$'s neighbors have also already received their advertisements for the round.
This latter property is necessary because it guarantees that if a node $u$ sends a connection invitation to neighbor $v$,
this neighbor has already received its advertisements for the round.

The third property requires for each node $u$ and round $r$,
that all connection behavior involving $u$ for round $r$ is complete before $u$ moves on to 
decide an advertisement for round $r+1$.
That is, not only has $u$ completed any attempted connections,
but all of $u$'s neighbors have also completed any attempted connections (including, importantly, connection invitations sent to $u$).

\paragraph{The MTM Sim Algorithm}
Our final step is to describe and analyze a strategy that implements the model interface and properties
described above using the MPC framework.
We call this strategy MTM sim (short for: mobile telephone model simulation).
We describe it below from
the perspective of a node $u$ that is using MTM sim to simulate some well-formed
mobile telephone model algorithm ${\cal A}$.



\begin{itemize}


%\begin{quote}{\bf simMTM Algorithm (simulating MTM for algorithm ${\cal A}$ on node $u$).}
\item At the beginning of each simulated round $r$,
the MTM sim algorithm calls the {\tt requestAdv}$(r)_u$ function implemented by ${\cal A}$ to learn $a_u(r)$: the advertisement generated by ${\cal A}$ for $u$ in simulated round $r$.
The algorithm updates $u$'s MPC framework advertisement to $\langle r, a_u(r), 0,0\rangle$.\footnote{We omit the requirement here for a node to include its
id in its advertisement. With the MPC framework you always learn the identify of the node that generated a discovered advertisement, so including it
in the advertisement payload is redundant.}

%The algorithm sets $u$'s advertisement to $\langle r, a_u(r), 0,0\rangle$.
%The first $0$ bit indicates (roughly speaking) that $u$ is not yet ready to end the scan phase of this round.
%The second $0$ bit indicates (roughly speaking) that $u$ is not yet ready to end the connect phase.

\item The MTM sim algorithm then blocks until it has learned the simulated round $r$ advertisement (i.e., as delivered in an MPC advertisement
 of  the form  $\langle r, *, *,*\rangle$) from each of $u$'s neighbors in the network.
At this point, the  algorithm does two things:  (1) it calls {\tt deliverAdv}$(r,A)_u$, where $A$ is the set of its neighbors'  advertisements for simulated $r$; and
  (2) it changes $u$'s MPC advertisement to $\langle r, a_u(r), 1,0\rangle$.

\item The MTM sim algorithm then blocks 
 until all of $u$'s neighbors have a $1$ in the third field of their MPC advertisement.
 At this point, it calls {\tt endScan}$(r)_u$.
 
 \item The MTM sim algorithm blocks until algorithm ${\cal A}$ running on $u$ calls {\tt endConnect}$(r)_u$. At this point,
MTM sim updates $u$'s MPC advertisement to $\langle r, a_u(r), 1,1\rangle$.
 
 \item The MTM sim algorithm blocks until all neighbors of $u$ include a $1$ in the fourth field of their MPC advertisement.
 At this point, it advances to simulated round $r+1$.
  
\end{itemize} 

Notice, it is possible that a node might miss an advertisement that it is waiting to receive during one of the blocking steps.
This can occur if a neighbor of some node $u$ changes its advertisement too quickly for $u$ to discover it.

To compensate for this possibility,
we assume our above algorithm {\em reconstructs} missed advertisements.
That is, if $u$ notices that it missed an advertisement from its neighbor $v$,
it reconstructs the missing advertisement based on the current advertisement it sees from $v$.
It then simulates first receiving the reconstructed advertisement before the current advertisement.
The core of the below correctness proof
is an argument that each node $u$ can fall behind at most one advertisement for a given neighbor.
A case analysis on the advertisement type then establishes that
 it is always possible to reconstruct the missed advertisement in this case.

\begin{theorem}
When executed with a well-formed  algorithm,
the MTM sim algorithm satisfies the mobile telephone model guarantees defined by Property~\ref{prop:mtm}.
%Furthermore, 
%for every round $r\geq 1$,
%node $u$,
%the MTM sim algorithm requires at most $O(r\cdot \hat t)$ time to simulate the first $r$ rounds for $u$,
%where $\hat t$ is the worst case time for a node to 
%
% = \delta_a + 2\delta_i + \delta_m$ is the round length.
\label{thm:mtm}
\end{theorem}
% [space cut]
\iffalse
\begin{proof}
We begin by studying MTM sim under the simplifying assumption
that no advertisements are missed.
That is,
if a node $u$ updates its advertisement to $a$, then all neighbors of $u$ learn of this update,
even if the interval between this update and $u$'s subsequent update is small.
Under this assumption,
the correctness of MTM sim is easy to establish as its operations directly implement the guarantees of Property~\ref{prop:mtm}.

As noted in the algorithm description, however,
it is possible that some advertisements are missed; e.g., $u$ updates to $a$, and then to $a'$ so fast
that some neighbor $v$ does not have enough time to discover $a$.
In this case, as described, the MTM sim algorithm attempts to reconstruct the missed advertisement.
To conclude this proof, we must show that this reconstruction is always possible,
which implies the nodes running MTM sim are simulating the above assumption of no missed advertisements.

To make this argument, we note that the we can place the MPC advertisement types used by MTM sim into a total order; i.e.,

\[ \langle 1, *, 0,0\rangle,  \langle 1, *, 1,0\rangle,  \langle 1, *, 1,1\rangle,\]  
\[\langle 2, *, 0,0\rangle,  \langle 2, *, 1,0\rangle, 
 \langle 2, *, 1,1\rangle, \langle 3, *, 0,0\rangle...\]

A useful property of the MTM sim algorithm is that if at a given point in an execution
a node $u$ is currently advertising the type in some position $i>1$ in the above total order,
then it must be the case that prior to this point all of $u$'s neighbors advertised the type in position $i-1$,
as this is required by the algorithm for $u$ to advance to the next advertisement type.

To apply this property, consider some node $v$ and some point in the execution
at which $v$ is advertising the type in some position $i \geq 1$.
For each neighbor $u$ of $v$,
$u$ can only be at most one advertisement type ahead of $v$. That is, it is possible that $u$
is advertising the type in position $i+1$ at this point, but it cannot be advertising
a type in a position strictly greater than $i+1$, as this would require a later advertisement type from $v$.
Furthermore, because $v$ is at position $i$, it must already know $u$'s type $i-1$ advertisement,
as this was required for $v$ to advance to position $i$.

In this case, it is possible that $v$ missed one advertisement from $u$.
That is, that $v$ missed $u$'s position $i$ advertisement as $u$ moved
from $i$ to $i+1$.
If this occurs $v$ will remain in $i$, and therefore $u$ will remain at type $i+1$,
until after $v$ is able to reconstruct $u$'s position $i$ advertisement.
It follows that $v$ will eventually hear $u$'s type $i+1$ advertisement and can use this to aid its reconstruction.

A simple case analysis on the advertisement types establishes that if $v$ knows $u$'s type $i-1$ advertisement
{\em and} its type $i+1$ advertisement, then $v$ has all of the information it needs
to reconstruct $u$'s type $i$ advertisement.
\end{proof}
\fi

We are left to bound the time complexity overhead generated by the MTM sim algorithm.
To do so, let the {\em round length} $\hat t$ be the worst case time required by the MPC framework
for any node to implement all three of the following steps: (1) update its advertisement and have all neighbors discover the update; (2) send a connection invitation
and have it accepted; and (3) send over the connection the bounded amount of information allowed in a single round of the mobile telephone model.
Clearly, $r\cdot \hat t$ is a worst-case lower bound on the time required to simulate $r$ mobile telephone model rounds,
as each such simulated round requires advertising, discovery, invitations, and (potentially) a connection.




\iffalse
%That is, we bound the worst case time required for a given node to complete the simulation of a given MTM round (i.e., the
%time between two consecutive {\tt requestAdv} calls). 

To do so, let $\delta_{m}$ be the maximum amount of time required to complete the bounded amount of communication
allowed during a connection in the MTM (this is a function of the bound on allowed communication and the slowest possible
bit rate $r_{max}$ at which this communication might occur). We define the {\em round length} $\hat t = \delta_a + 2\delta_i + \delta_m$.
(Recall from Section~\ref{sec:pmtm} that $\delta_a$ and $\delta_b$ are the maximum times to 
spread a new advertisement to all your neighbors and send/reply to a connection attempt, respectively.)

The round length $\hat t$ is therefore the worst case time required for a pair of nodes to hear each others' advertisements and then
form a connection. 
It follows that $\hat t$ provides an obvious lower bound for the worst case time required to simulate a given round of the MTM model.
Here we prove that in the worst case, simMTM requires $O(r\cdot \hat t)$ time to simulate $r$ rounds; i.e., 
the average time per round is within a constant factor of the obvious lower bound.\footnote{We emphasize that this result 
is not necessarily expected. The simMTM algorithm requires nodes to collect advertisements of a certain type from
all of their neighbors before moving on to the next type. It is plausible, therefore, the network might generate over time a chain
of dependencies. For example, imagine a line network in which we label the nodes $1,2,3...,n$. Imagine each node $i >1$
is waiting on an advertisement from its neighbor $i-1$ of the type in position $i-1$ of the total ordering used
in the proof of Theorem~\ref{thm:mtm}. This creates a chain of dependencies until we have to wait for
$i$ to update its type before $i+1$. The total time until node $n$ makes progress, therefore, is now a function
of the network size. We leverage a classical result from the study of synchronizers to show such chains
take a long time to establish and the average time per round therefore remains efficient.}
\fi

Our goal is to prove that the MTM sim strategy matches this lower bound within constant factors.
Fortunately, this property follows by noting that the advertisement blocking implemented by MTM sim is a standard
local synchronization strategy, and then applying the
 classical results on local synchronization first implied by Gallager~\cite{gallager:1982} and Awerbuch~\cite{awerbuch:1985},
 and later formalized by Lynch~\cite{nancytextbook} in  Section 16.2). Formally:



%a simple synchronizer strategy in which nodes in an asynchronous message passing model must send and collect
%round $i$ messages from each neighbor before sending a round $i+1$ message, requires, for each count $r\geq 1$,
%$O(r(d+\ell))$ time to get all nodes up to round $r$,
%where $d$ is an upper bound on message delay and $\ell$ is an upper bound on the 
%ocal steps at a given node required for each round.

%By equating each advertisement type as a round in the classical synchronizer
%result, and noting in this context the delay between subsequent advertisement types is bounded by $O(\hat t)$, implying $d+\ell = O(\hat t)$, 
%the following holds:

\begin{theorem}
For any $r\geq 1$,
node $u$, and MPC round length $\hat t$,
the MTM sim algorithm requires $O(r\cdot \hat t)$ time to simulate the first $r$ rounds for $u$.
\label{thm:time}
\end{theorem}


\paragraph{Tolerating Network Changes}
We conclude by noting that the MTM sim algorithm as described is not particularly fault-tolerant.
If a neighbor of $u$ crashes or leaves the area, for example, 
$u$ will block indefinitely waiting for $u$'s next anticipated advertisement type.
A straightforward heuristic to accommodate this possibility is to implement a simple time out mechanism: if $u$ fails
to hear from neighbor $v$ for sufficiently long, $u$ removes $v$ from its list of neighbors.


Similarly, if node $u$ hears an advertisement of a {\em new} neighbor $v$,
it can add $v$ to its neighbor list starting with an upcoming round.
If node $v$ was a neighbor that $u$ recently removed due to a time out, it might conclude that
its time out value is too small and increase it---allowing it to adapt to the current network conditions.
%
More generally, we note that identifying optimal heuristics for tolerating network changes is important
future work to help advance this research direction.

\iffalse

Finally, we note that when a node $u$ joins a network for the first time,
or migrates from one network partition to another,
it might discover that its new neighbors are far ahead or behind in their rounds. 
In this case, $u$ can make a discontinuous jump to the local round to allow it to proceed with it neighbors going forward.
It might therefore make sense in this case to add a {\tt roundAdjust}$(r,r')$ function to the mobile telephone model interface
to provide algorithms a way to be notified that a round jump occurred.
Such jumps have little effect on our random spread gossip algorithm,
but other algorithms might require specific action to recover from such changes.

We leave the details of identifying the best possible modifications to MTM sim to tolerate changing networks
as interesting future work. 

\fi







